Tuning the Tail Latency of Distributed Queries Using Replication

Querying graph data with low latency is an important requirement in application domains such as social networks and knowledge graphs. Graph queries perform multiple hops between vertices. When data is partitioned and stored across multiple servers, queries executing at one server often need to hop to vertices stored by another server. Such distributed traversals represent a performance bottleneck for low-latency queries. To reduce query latency, one can replicate remote data to make distributed traversals unnecessary, but replication is expensive and should be minimized. In this paper, we introduce the problem of finding data replication schemes that satisfy arbitrary user-defined query latency constraints with minimal replication cost. We propose a novel workload model to express data access causality, propose a family of heuristics, and introduce non-trivial sufficient conditions for their correctness. Our evaluation on two representative benchmarks show that our algorithms enable fine-tuning query latency with data replication and can find sweet spots in the latency/replication design space.

==> __latexindent_temp.tex <==
\section{Proposed algorithm}


\begin{algorithm}
\centering
\caption{Baseline Algorithm}\label{algo:baseline}
\begin{flushleft}
\hspace*{\algorithmicindent} \textbf{Input: } Query types $Q_t$, hop budget $k$,\\ data partitioning scheme $P : v \longrightarrow \{ s_1, s_2, ..., s_i \}$\\
\hspace*{\algorithmicindent} \textbf{Output: } Replication Scheme $R : v \longrightarrow \{ s_1, s_2, ..., s_i \}$
\end{flushleft}
\begin{algorithmic}[1]
\State $R \gets \{\}$
\For{query type $q_t \in Q_t$}
    \For{$v \in$ all possible starting vertices $q_t.V$}
        \State $H$ =  \Call{to\_hypergraph}{$v, q_t, P$}
        \For{path $p \in H$}
            \If{$p.length > k$}
                \State $h_j = h \in p$ with height $k$  
                \For{$h_i \in p$ where $h_i.height > k$}
                    \State $R \gets R \cup h_i.V \longrightarrow h_j.s$
                    \If{$i - j > 1$ and $h_j \neq h_{root}$}
                        \For{$n \in range(j+1, i)$}
                            \State $R \gets R \cup h_i.V \longrightarrow h_n.s$
                        \EndFor
                    \EndIf
                \EndFor
            \EndIf
        \EndFor
    \EndFor
\EndFor
\Return $R$
\end{algorithmic}
\end{algorithm}



With the cascading replication constraint, we present the proposed baseline algorithm in figure \ref{algo:baseline}.  
\nn{explain proposed baseline}

Instead of replicating layers that violates the $k$-layer guarantee to the $k^{th}$ layer of the causal access tree, one straight forward way to improve the algorithm is to explore other possible plans under the replication constraints to minimize the replication cost.
We present the proposed algorithm in figure \ref{fig:proposed_algo_1}.



\begin{algorithm}
\centering
\caption{Local\_min Algorithm}\label{algo:local_min}
\begin{flushleft}
\hspace*{\algorithmicindent} \textbf{Input: } Query types $Q_t$, hop budget $k$,\\ data partitioning scheme $P : v \longrightarrow \{ s_1, s_2, ..., s_i \}$, \\
data size map $M : v \longrightarrow size(v)$\\ 
\hspace*{\algorithmicindent} \textbf{Output: } Replication Scheme $R : v \longrightarrow \{ s_1, s_2, ..., s_i \}$
\end{flushleft}
\begin{algorithmic}[1]
\State $R \gets \{\}$
\For{query type $q_t \in Q_t$}
    \For{$v \in$ all possible starting vertices $q_t.V$}
        \State $H$ =  \Call{to\_hypergraph}{$v, q_t, P$}
        \For{path $p \in H$}
            \If{$p.length > k$}
                \State Plans $\mathcal{P} = $ \Call{enumerate\_plans}{$p$}
                \State $R \gets R$ $\cup$ \Call{get\_min\_plan}{$\mathcal{P}, P, R, M$}
            \EndIf
        \EndFor
    \EndFor
\EndFor
\Return $R$
\end{algorithmic}
\end{algorithm}

\textbf{Upper bound of the number of possible replication schemes. }
With the upward replication constraint and layer-based replication constraint, the upper bound of the number of possible replication scheme given an $n$-hop query and a budget $k$ is $\ceil*{n - 1 \choose k - 1}$, where all data accesses after processing the root result in an inter-server communication. 
With our query routing logic, the first layer of the $n$-hop query is always a chosen layer. 
For the remaining $n - 1$ layers, we can choose $k - 1$ layers as the chosen layer, and replicate other nodes in other non-chosen layers to it's closest chosen layer parent. 
Therefore, the upper bound of the number of possible replication scheme for an $n$-hop query and a budget $k$ is $\ceil*{n - 1 \choose k - 1}$. 

\nn{second argument - We can do this cost computing in parallel (multi-thread). So even if there are lots of plans to compute it will be fine. }

\subsection{Example of poor proposed algorithm}

In practice, we notice that picking the plan with the local minimum replication cost does not necessarily leads to the global minimum replication cost. 
It is because the decision ignores the \emph{data dependency} between hops. 
We use Figure \ref{fig:short_q_7} to illustrate the idea. 

\begin{figure}[]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/short_query_7.png}
    \caption{SNB short query type 7. }
    \label{fig:short_q_7}
\end{figure}

Figure \ref{fig:short_q_7} shows the query structure of the SNB short query type 7. 
Given a starting $Message$, get all the $Comment$ reply to the $Message$, and get the $Person$ that creates the $Comment$ (i.e., $Message \rightarrow Comment \rightarrow Person$).
Assume that all hops locate at a different server, hence $k = 3$ if no replica exists, and suppose the goal is to provide a 2-layer guarantee. 
Consider the query path $Message \rightarrow Comment_1 \rightarrow Person_1$. 
The proposed baseline algorithm will replicate all vertices that violates the 2-layer guarantee ($Person_1$) to the $2^{th}$ layer ($Comment_1$). 
Our proposed algorithm will enumerate all the possible plans under the two replication constraint (i.e., upward replication constraint and "follow the parent" constraint), and replicate according to the plan with the local minimum replication cost, where the replication cost is calculated by $sum(size(replicas\ created))$.  
Since the size of $Comment_1$ is smaller than the size of $Person_1$ vertex, our replication algorithm will replicate the $Comment_1$ to the $Message$ server. 

In the example in Figure \ref{fig:short_q_7}, each $Comment$ will only reply to one $Message$ (i.e., 1-many relationship between $Message$ and $Comment$), which means that each $Comment$ vertex will only appear in only one query execution path, and replicating $Comment$ will only minimize the communication cost for one query path. 
On the other hand, a $Person$ may create multiple $Comment$ (many-to-1 relationship between $Comment$ and $Person$), and replicating $Person$ to $Comment$ may potentially not only minimize the communication cost for the current query path, but also other query paths. 
For example, replicating $Person 1$ to $S_2$ can optimize both $Message \rightarrow Comment_1 \rightarrow Person_1$ and $Message \rightarrow Comment_2 \rightarrow Person_1$. 
This specific example shows that a better cost model is needed to capture the data dependencies between hops. 

\subsection{Proposed cost model}
To incorporate the data dependencies between hops, we propose a cost model to compute the replication cost given a replication scheme for a causal access tree. 
The intuition of our cost model is to split the cost of replicating a vertex to consider other query paths that include the vertex. 
Specifically, given a replication plan $v \rightarrow S_i$, the cost of replicating $v$ to $S_i$ is 
\[
    cost(v, S_i)= 
\begin{cases}
    0,& \text{if } v' \in S_i\\
    \frac{size(v)}{|parent(v) \in S_i|}, & \text{otherwise}
\end{cases}
\]
There are two cases in the cost model. 
If $v$'s replica ($v'$) already exists in $S_i$, there is no need for new replication thus the cost is 0. 
Otherwise, the cost of replicating $v$ to $S_i$ equals to the size of $v$ divided by the number of path that it is potentially co-optimizing (i.e., $|parent(v) \in S_i|$). 

Consider the above example, for query path $Message \rightarrow Comment_1 \rightarrow Person_1$, the original cost of replicating $Person_1$ to $S_2$ is $cost_{original}(Person_1, S_2) = size(Person_1)$, and the cost of replicating $Comment_1$ to $S_1$ is $cost_{original}(Comment_1, S_1) = size(Comment_1)$. 
Since $size(Comment_1) < size(Person_1)$, our original replication algorithm will replicate $Comment_1$ to $S_1$. 

With our proposed cost model, $cost_{proposed}(Person_1, S_2) = \frac{size(Person_1)}{2}$, since it optimize for both $Message \rightarrow Comment_1 \rightarrow Person_1$ and $Message \rightarrow Comment_2 \rightarrow Person_1$. 
With our proposed cost model, we empirically shows that it can achieve a lower overall replication cost. 

\[
    cost(v, S_i)= 
\begin{cases}
    0,& \text{if } v' \in S_i\\
    \frac{size(v)  + \alpha M_i}{|parent(v) \in S_i|}, & \text{otherwise}
\end{cases}
\]

, where user-defined $\alpha$ is a parameter and $M_i$ is the current memory utilization of server $S_i$.

$M_i$ can be the number of replicas we created in $S_i$

\nn{just changed the cost model in proposed algorithm

\nn{multithreading can also be enabled since we use a simple routing mechanism. 
The routing logic does not have to be included into the replication table, such that we can simple use a binary array to indicate the replication scheme, and avoid locking. }
\ref{fig:proposed_algo_1}. No need to add another algorithm here? }

==> algorithms/naive-robust.tex <==
\caption{Robust Replication Algorithm}\label{algo:cascading_proof}
\begin{algorithmic}[1]
    \Procedure{update}{$r, p, t$}
        \State \emph{budget} $\gets t$
        \State $n \gets$ length($p$)
        \For{$i \gets 1$ to $n-1$}
            \State \emph{budget} $=$ \emph{budget}$- l(d(v_{p_i}),d(v_{p_{i+1}}))$
            \If{$d(v_{p_i}) \neq d(v_{p_{i+1}})$}
                \State \emph{index} $= i + 1$
            \EndIf
            \If{\emph{budget}$< 0$}
                \For{$j \gets i+1$ to $n$}
                    \State $r(v_{p_j}) \gets r(v_{p_j}) \cup d(v_{p_i})$
                    \For{$k \gets index $ to $j - 1$}
                        \State $r(v_{p_j}) \gets r(v_{p_j}) \cup d(v_{p_k})$
                    \EndFor
                \EndFor
                \State \textbf{break}
            \EndIf
        \EndFor
        \Return $r$
    \EndProcedure
\end{algorithmic}

==> algorithms/naive.tex <==
\centering
\caption{Na\"{i}ve Replication Algorithm}\label{algo:naive}
\begin{algorithmic}[1]
\Procedure{update}{$r, p, l, t_Q, f, \epsilon$}
    \State \emph{budget} $\gets t_Q$
    \State $n \gets$ length($p$) \Comment{$p = \langle v_{p_1}, \ldots, v_{p_n}\rangle$}
    \For{$i \gets 1$ to $n-1$}
        \State \emph{budget} $=$ \emph{budget} $- l(a_{C,r}(v_{p_i}),a_{C,r}(v_{p_{i+1}}))$
        \If{\emph{budget} $< 0$}
            \For{$j \gets i+1$ to $n$}
                \State $r(v_{p_j}) \gets r(v_{p_j}) \cup \{a_{C,r}(v_{p_i})\}$
            \EndFor
            \State \textbf{break}
        \EndIf
    \EndFor
    \If{$\exists s, s' \in S:\: |f_r(s) - f_r(s')| > \epsilon $}
        \State{\Return \emph{no-solution-found}}
    \EndIf
    \State{\Return $r$}
\EndProcedure
\end{algorithmic}


==> algorithms/optimized.tex <==
\caption{Proposed Replication Algorithm}\label{algo:proposed_old}
\begin{flushleft}
    \hspace*{\algorithmicindent} \textbf{Input: } 
    a set of query matches $\mathcal{M}$, 
    a set of matched causal access trees $\mathcal{C_M}$, 
    data placement function $d$, 
    replicated data placement function $r$, 
    a latency function $l$, 
    and a set of latency budget $T$ for each match in $\mathcal{M}$\\
    \hspace*{\algorithmicindent} \textbf{Output: } updated replicated data placement function $r'$
\end{flushleft}
\begin{algorithmic}[1]
\State $r' \gets r$
\For{$M \in \mathcal{M}$}
    \State computed subpaths $CS \gets \{\}$
    \State $P_M \gets$ all root-to-leaf paths in $C_M$
    \For{$p:\{v_1, v_2, ...,v_n\} \in P_M$}
        \If{$\langle p.v_1.s, p.v_2 \rangle$ $\not\in CS$}
            \State $m_p \gets []$
            \State $m_p.append([v_1])$
            \For{$i \gets 2$ to $n$}
                \If{$d(v_{i-1}) \neq d(v_i)$}
                    \State $m_p.append([v_i])$
                \Else
                    \State $m_p[m_p.size].append(v_i)$
                \EndIf
            \EndFor
            \State $CS \gets$ all subsets of $m_p[2:]$ of size $T(M)-1$
            \State $min\_cost\_plan = \emptyset$ 
            \For{$c \in C$}
                \State $c \gets 1$
                \State $c.cost = 0$
                \For{$i \gets 2$ to $m_p.size$}
                    \If{$m_p[i] \not\in c$}
                        \State $m_p[j] \gets$ closest $m_p \in c$
                        \For{$v \in m_p[i]$}
                            \For{$k \gets j$ to $i - 1$}
                                \State $c.cost += COST(v, d(m_p[k][0]), M)$
                            \EndFor
                        \EndFor
                    \EndIf
                \EndFor
                \If{$c.cost < min\_cost\_plan.cost$}
                    \State $min\_cost\_plan = c$
                \EndIf
            \EndFor
            \For{$i \gets 2$ to $m_p.size$}
                \If{$m_p[i] \not\in min\_cost\_plan$}
                    \State $m_p[j] \gets$ closest $m_p \in min\_cost\_plan$
                    \For{$v \in m_p[i]$}
                        \For{$k \gets j$ to $i - 1$}
                            \If{$d(m_p[k][0]) \not\in r(v)$}
                                \State $r'(v) \gets r'(v) \cup d(m_p[k][0])$
                            \EndIf
                        \EndFor
                    \EndFor
                \EndIf
            \EndFor 
        \EndIf
        \State $CS \gets CS \cup \langle p.v_1.s, p.v_2 \rangle$
    \EndFor        
\EndFor
\Return $r'$

\end{algorithmic}






==> sections/Introduction-SIGMOD.tex <==
\section{Introduction}
In many important domains, such as social media, search engines, and question answering (Q\&A) systems, it is common to model structured data as a graph.
Applications in these domains often operate on large graphs stored on a distributed system and require end-to-end query latencies in the order of milliseconds~\cite{A1,tao,unicorn,Wukong,Pragh,social_hash,linkbench,trinity_rdf,chiller,managing_large_dynamic_graphs_efficiently,DistDGL}.
Graph queries are in the critical path of several user-facing production applications, where they must complete within a fixed low-latency constraint. 
%, in the order of milliseconds.
For example, Facebook uses a graph to represent critical data such as users, posts, or comments, and queries the graph to render web pages and to serve user searches~\cite{tao,linkbench,unicorn}.
The Bing search engine queries its knowledge graph to render pages~\cite{A1}.
Q\&A systems powering Amazon's and Alibaba's personal assistants query their knowledge graphs~\cite{ubiquity}.
To support low-latency graph queries, several distributed in-memory graph data management systems have been proposed and used in production~\cite{trinity, tao, trinity_rdf, A1, Wukong, Pragh, gtran, grasper, neo4j_linkedin}.

Ensuring that graph queries reliably respect their mandated low-latency constraint is challenging.
Graph queries perform multiple hops to iteratively traverse edges.
When the graph is partitioned and stored across distributed servers, a query executing at a server may require \emph{distributed traversals}, that is, traverse edges to destination vertices stored by other servers.
%In this case, to move compute to data, the query executor needs to send the unprocessed hops of the query (a.k.a. subquery) to that server to continue the processing. 
Distributed traversals represent the main performance bottleneck in low-latency multi-hop queries.
Prior work has shown that data access locality is critical for performance: local accesses are 20x-100x faster than remote accesses, even with advanced networking technologies such as Remote Direct Memory Access~\cite{A1,Pragh,Wukong,gtran,grasper}.
Distributed traversals can be eliminated using replication, but this introduces an extra storage cost, which is undesirable, especially in in-memory storage systems.

In this paper, we address for the first time the following question:
% for low-latency multi-hop query workloads: 
\emph{how to meet an arbitrary user-specified query latency  constraint while minimizing data replication?}
Constraining latency requires reasoning in terms of the worst-case access paths of a query.
We formalize this as an optimization problem where the query workload is modeled as \emph{causal access trees} representing the causal relationship among data accesses.
The latency of a query is then represented by its slowest chain of causally-dependent data accesses, which must be performed sequentially.
This formalism can model any query having a multi-hop access pattern, independent of how queries are expressed (i.e., using a relational or graph query language) and how the data is stored (i.e., using a relational or a graph-native database).
%\nn{represented or stored? Should be structured (relational) or unstructured (graph)?}.
%The system model pushes subqueries to remote servers to maximize query locality and replication flexibility, rather than fetching data. 
%We also model and implement graph query executors that maximize query locality and leverage data replication by pushing subqueries to remote servers, rather than fetching data.
Navigating the space of solutions to this problem introduces a number of novel and interesting technical challenges.

We first investigate \emph{distributed query routing}.
Data replication gives rise to a huge number of possible query access paths.
A distributed traversal could be directed any remote copy of the required data, and different queries of a workload may have to access different copies to meet their latency requirements.
Keeping track of the mapping between queries and optimal data locations requires additional routing tables that could be unfeasibly large.
To avoid this problem, we define a class of replication schemes called \emph{upward replication functions} and formally prove that they have minimal replication cost when queries are executed without additional routing tables storing the location of replicas.

\begin{figure*}[t!]
  \centering
  \begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/hop_vs_latency.pdf}
    \caption{Per-query latency with varying number of distributed traversals required}
    \label{fig:hop_vs_latency}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.21\textwidth}
      \centering
      \includegraphics[width=\textwidth]{figures/short_queries_remote_per_q_CDF_hash.pdf}
      \caption{CDF of distributed traversals required per query with hash partitioning.}
      \label{fig:remote_per_q_hash}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.21\textwidth}
      \centering
      \includegraphics[width=\textwidth]{figures/short_queries_remote_per_q_CDF_metis.pdf}
      \caption{CDF of distributed traversals required per query with min-cut partitioning.}
      \label{fig:remote_per_q_metis}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/k0_replication_cost.pdf}
    \caption{Replication overhead to guarantee 0-traversals with different data placements.}
    \label{fig:k0_replication_cost}
  \end{subfigure}
  \label{fig:short_queries_remote_per_q}
  \vspace{-0.5\baselineskip}
  \caption{Distributed multi-hop queries in the LDBC SNB interactive workload.}
  \vspace{-0.5em}
\end{figure*}

We then propose \emph{replication algorithms} that provide arbitrary latency guarantees while minimizing replication cost given a multi-hop query workload.
Data accesses often overlap across queries in a workload, and co-optimizing replication across a large number of queries may be unfeasible. 
We describe a family of greedy algorithms that analyze a subset of the query workload at a time and greedily add new data replicas to enforce the latency constraints on that subset.
We show that writing correct greedy replication algorithms is not straightforward.
Greedily adding new replicas may introduce violations of the latency constraint of some previously optimized queries.
We formally prove sufficient conditions that, if enforced by the replication algorithm, can avoid such problems.
%In some workloads, it is necessary to deal with \emph{dynamic updates} to the graph, for example, to add vertices and edges.
Finally, we propose correct replication algorithms for both \emph{static and dynamic} graphs.

% Using replication to reduce data access latency is a recurrent topic in distributed computing, but no prior work has considered the problem of enforcing arbitrary latency bounds on multi-hop queries.
% SPAR uses data replication to ensure that there are no distributed traversals when executing $1$-hop graph queries~\cite{SPAR}. 
% Finding replication schemes that eliminate distributed traversals even in the general case of $n$-hop queries is simple, but it leads to high replication costs, as we show in this paper. 
% This work enables a more flexible tuning of the latency bound to reduce the replication cost.
% This results in a much larger design space and a more challenging optimization problem.
% Other work proposed data replication heuristics that can be used to reduce query latency.
% For example, one could replicate all the neighbors of a vertex at the same server \cite{Wukong,DistDGL}. 
% This replication schemes can be seen as enforcing a specific latency bound: if $n$ is the number of hops in the query, then this replication scheme ensures an upper bound of  a $\lfloor n/2 \rfloor$-traversal guarantee for queries, where . 
% This generalization results in a significantly more challenging problem, which needs to consider not only the graph structure but also the query workload.
%However, this approach is workload-unaware, which results in higher replication cost than our workload-aware approach, as we show in our evaluation. 
%Also, in both approaches, users do not have control on both the query latencies and the replication cost as existing algorithms are designed to generate replication schemes for only a specific traversal guarantee. 

We evaluate our algorithms using two diverse graph query benchmarks.
The first is the LDBC Social Network Benchmark "interactive short queries" workload, the standard benchmark for low-latency user-facing graph query workloads~\cite{ldbc}.
The second is node-wise neighborhood sampling, a critical bottleneck for distributed mini-batch training of Graph Neural Networks (GNNs)~\cite{DistDGL}. 
%To show the generality of the approach, we also consider a different type of workload: distributed node-wise neighborhood sampling for Graph Neural Network training over graphs from the Open Graph Benchmark \cite{OGB}.
%We consider neighborhood sampling as the workload, which is performed online at each training iteration to obtain mini-batches \cite{DistDGL}. 
%Distributed GNN training systems like DistDGL perform distributed graph sampling online at each training iteration to obtain mini-batches \cite{DistDGL}.
%To reduce GNN training time, sampling must be efficient \cite{nextdoor, case}.
%We show that the replication criteria used in DistDGL can be seen as a special case of our framework and that our algorithms can achieve a lower replication cost compared to DistDGL.
Our evaluation shows that our algorithms enable fine-tuning query latency (both average and tail) and trading latency guarantees with data replication cost.
Setting the latency constraints in these workloads can vary the query latency by a factor of up to $120\times$ and the overall storage cost by up to $3\times$.
It is therefore critical to fine-tune this parameter to find the right latency-replication tradeoff.
%Our selective data replication algorithms enable users to control both average and tail latency.
%We find that by relaxing the latency bound to allow some amount of traversals, we can significantly reduce the replication cost while still being able to control query latencies
In both workloads, we found that there exists a sweet spot in this tradeoff: relaxing the latency constraint reduces replication cost until we reach the sweet spot, then further relaxations have diminishing returns.
We show that controlling latency constraints also enables controlling throughput.
Our algorithms can accommodate dynamic updates to the graph with a low replication cost. 
%In GNN sampling workloads, our algorithms can achieve the same latency guarantees as DistDGL's replication scheme with lower replication cost. \nn{remove this and not stress this part?}
Finally, our algorithms are efficient and practical: they can generate a replication scheme for billion-scale graphs in less than 22 minutes.

In summary, our key contributions are: 
%\setlist{nolistsep}
\begin{itemize}[parsep=1.5pt,topsep=1.5pt]
  \item We formalize the \emph{latency-bound replication problem}, which characterizes a large and complex design space.
  \item We characterize a class of replication schemes that are optimal when no additional routing information is introduced.
  \item We show that writing greedy replication algorithms are not straightforward and formally prove sufficient correctness conditions for the replication scheme.
  \item We propose replication algorithms for both static and dynamic graphs.
  \item We empirically validate our algorithms using two diverse query workloads.
\end{itemize}
%\setlist{nolistsep}
\vspace{-1em}
\section{Background and Motivation}
%During query processing, when the required next-hop vertex does not exist in the local storage, the query executor needs to route the query to another server that contains the target data, which results in a \emph{distributed traversal} from one server to another.  
We first present some observations about the performance of low-latency multi-hop queries that motivate our work and formal model.
We focus on the interactive short read query workload of the LDBC Social Network Benchmark (SNB)~\cite{ldbc}.

\spara{The distributed traversal bottleneck in multi-hop queries}
Low-latency distributed multi-hop queries are bottlenecked by the number of consecutive distributed traversals required to process them.
Figure~\ref{fig:hop_vs_latency} shows that as the number of distributed traversals required to process a query grows, the query latency grows almost linearly, and this holds for both average and tail latency.

The number of distributed traversals required may be large, depending on the data placement scheme. 
Figure~\ref{fig:remote_per_q_hash} and ~\ref{fig:remote_per_q_metis} shows the CDF of the number of distributed traversals required per query with varying numbers of servers in the system.
With distributed hash partitioning, which is commonly used by in-memory graph databases such as A1~\cite{A1} and Wukong~\cite{Wukong}, 30-40\% of queries require more than one traversal (see Figure~\ref{fig:remote_per_q_hash}). 
Note that the number of distributed traversals can be larger than the number of servers since a query may traverse between two servers multiple times.
Using an offline min-cut partitioning algorithm such as Metis~\cite{METIS} to partition the data graph while minimizing edge cuts across servers can reduce the number of distributed traversals, as shown in Figure~\ref{fig:remote_per_q_metis}. 
However, even with this computationally costly offline optimization, there still exists a long tail of queries that require a large amount of distributed traversals.

\spara{The importance of flexible latency constraints}
Using data replication can reduce the number of distributed traversals required per query as it replaces distributed traversals with local accesses to local replicas. 
One simple approach to constrain latency would be to replicate data until no distributed traversal is necessary for any query. % (a.k.a., providing a $0$-traversal guarantee) \cite{SPAR}. 
We argue that providing this level of guarantee requires a high replication cost, even when using a replication algorithm that analyzes a known workload and replicates the minimum amount of data.
We support this claim through the following experiment.
Given a known SNB workload, we replicate all remote data required by each query to the server that stores the master copy of the starting vertex of the query, such that subsequent data required can be found locally at that server. 
We report the replication overhead of the system when using the two above mentioned data placement schemes in Figure \ref{fig:k0_replication_cost}. 
In the best case, the system still has to store twice as much data as the original graph in a cluster of six servers. 
%Online data migration can avoid this replication cost, but it is not commonly used since it introduces data transfer overheads and requires dedicated system support~\cite{MorphoSys,Pragh}.

In this paper, we propose algorithms to constrain the number of distributed traversals required by each query $Q$ to $t_Q$, where $t_Q$ is a tunable parameter and is query-specific.
Our work enables users to tune the query latency with respect to their replication budget.
We also show that by relaxing the latency constraints, we can substantially reduce the replication cost. 



\begin{comment}
\spara{Existing replication approaches}
There have been various attempts to alleviate the network burden of distributed queries by leveraging data replication.
Schism \cite{schism} is a workload-aware data partitioning algorithm that aims to minimize the number of distributed transactions.
It uses a set of offline workload traces to generate a data partitioning scheme and a replication scheme.
However, it does not provide the flexibility for users to bound the latency cost. 
SPAR \cite{SPAR} and MorphoSys \cite{MorphoSys} provide a \emph{guarantee} on the number of server hops each query requires. 
SPAR guarantees all the 1-hop queries will only need to access one server to retrieve required data by proposing replication policies. 
In this case, the inter-server communication cost is reduced to 0 (i.e., no distributed accesses). 
However, SPAR only provides a \emph{0}-hop guarantee for 1-hop queries, and the algorithm cannot be naturally extended to multi-hop queries, which is a key type of operation in practice. 
MorphoSys provides a \emph{0}-hop guarantee for all queries by altering its physical design before query execution. 
Nevertheless, MorphoSys optimizes for transactional workloads, which primarily consist of range scans.
It assumes that the read set and write set of a query are known before the actual query execution. 
This assumption does not hold for graph workloads, as the next hop of a query is decided based on the previous hop and will not be known until query execution time. 
Moreover, MorphoSys does not provide a flexible latency budget for different queries. 


\section{Scrap text}

We formalize this problem as an optimization problem and show that solving 




\subsection{snippets here and there}
\spara{Applications that need low-latency graph queries}
Graph traversal (aka multi-hop or graph-walking) queries have been prevalent and important operations atop graph store to support emerging applications like fraud detection in ecommerce transaction, user profiling in social networking, query answering in knowledge base, and urban monitoring in smart city. (Section 1 in Pragh)

The Bing search engine handles massive amounts of unstructured and structured data. To efficiently query the structured data, we need a platform that handles the scale of data as well as the strict performance and latency requirements. (Section 1 first sentence in A1)

LinkedIn's economic graph database is a very high performance graph query system designed for low latency queries similar to A1. It scales up vertically and can answer lookup queries in nanoseconds while A1 operates in microseconds. (Section 8 in A1)

Graph analytics has a broad spectrum of applications in industry. Recently, a large number of graph processing systems have been proposed (e.g., Pregel, PowerGraph), which support efficient offline graph computation such as PageRank, BFS, and connected components. However, processing online graph analytical queries (or OLAP) remains to be challenging since it has much stricter requirements on both latency and throughput. (Section 1 in Grasper)
\newline

\spara{Other systems that tried to target this use case}
\subsubsection{They use RPC}
Operators like predicate evaluation and edge enumeration are shipped to the machine hosting the vertex via RPC so that it can be evaluated without invoking a remote read. When we have multiple vertex operators to be processed at the same machine, we batch the operators together per machine to reduce the number of RPCs. (Section 3.4 in A1)

We currently place vertices randomly across the whole cluster and use locality to push query execution to where data resides. Looking at sample query executions, we have found that this strategy can be highly effective (95\% local reads) and we will discuss more in section 6. (The end of Section 3.2 in A1)

\subsubsection{They care about locality}
Graph traversal workloads are severely sensitive to the access locality, while it is notoriously difficult to partition graph with good locality. For example, the difference of median latency for two-hop query (like friends-of-friends (FoF) [18]) over a Graph500dataset (RMAT26)[12] is about 30× (0.75ms vs. 22.5ms) between a single machine and an 8-nodecluster. (Section 1 in Pragh)

The whole section 2.2 in Pragh studies how locality affects throughput and latency. 

RDMA reduces latency, but there is still a 20x - 100x difference between accessing local memory vs. remote memory. (Section 2.2 in A1)

Wukong may duplicate edges to make sure each machine contains a self-contained subgraph (e.g., no dangling edges) of the input RDF graph, for better locality. (Section 3 in Wukong)

future work in Social hash: incorporating alternative replication schemes for further reducing fanout in storage sharded systems. (Section 8)

Due to the power-law distribution on vertex degree and the small world phenomenon of most real-world graphs, the cost of traversal-based queries can be very high after multi-hops (e.g., >= 2) fan-out (Section 3 in G-Tran)

\subsection{Background}

Graph data analysis is a key operation to derive knowledge from real-world graphs.
For instance, one may explore and discover connections and patterns in a social network to recommend friends, products, or posts. 
As the graphs' sizes grow continuously, multiple machines are needed to fit the graph. 
There are many ways to represent and query graphs, ranging from dedicated graph databases to traditional relational databases. 
Even if the technologies might differ, the fundamental challenges of executing efficient distributed graphs queries are the same.

In a distributed environment, the properties of graph workloads can substantially reduce single-server optimizations. 
Specifically, graph workloads consist of complex, irregular random access patterns consisting of multiple hops. 
This characteristic increases the chance that a query needs to contact multiple servers to retrieve the query result. 
Hopping across various servers will introduce costly inter-server communications and data transfer, increasing the system's latency and network traffic and lowering the system's throughput. 
We use Figure \ref{fig:multihop_example} and \ref{fig:causal_access_tree} as an example to illustrate the idea.
Figure \ref{fig:multihop_example} shows a general example of a multi-hop query. 

In the example query, given a starting vertex $person_1$, the query traverses to all $person_1$'s friends ($1^{st}$ hops) through the \emph{knows} edges of $person_1$, 
and then from each $1^{st}$ hops, 
traverses to the $message$ vertices through each $1^{st}$ hop's corresponding \emph{creates} edges. 
The data accesses by this example query can be represented as a directed graph, depicted in Figure \ref{fig:causal_access_tree}.
In this graph, each vertex represents a data vertex the query accessed, and each directed edge $E(v_1, v_2)$ denotes the causal relationship between the two vertices. 
That is, $v_2$ is required and are only known after the processing of $v_1$. 
For example, we do not know which $2^{nd}$ hop $message$ are required before processing each of the $1^{st}$ hop $person$. 
The exampe query starts at the server ($s_1$) that contains $perosn_1$, and retrieve the neighbbor list of $person_1$ to get the set of next hop vertices ($1^{st}$ hop, $person_2$ and $person_3$). 
Since $person_3$ exists at $s_1$, the query can continue to process the next hop locally. 
However, as $s_1$ does not contain $person_2$, the sub-query ($person \rightarrow message$) needs to be routed to the server $s_2$ that contains the next hop vertex ($person_2$). 
We denote inter-server communications as red directed edge, and local next hop processing as black directed edge. 
For low latency queries, such inter-server traversal may become the bottleneck of processing the query. 
In particular, although local query processing (vertices in different root-to-leaf path) can be done in parallel on mutliple servers (e.g., retrieving $message_5$ and $message_6$), the causal access (vertices in the same root-to-leaf path) are happened sequentially (e.g., retrieving $person_1$ and $person_2$). 
In this case, the latency of the query equals to the path from root to leaf that contains the most number of inter-server hops (i.e., $person_1 \rightarrow person_2 \rightarrow message_5$).
Note that the length of the critical path may be larger than the total number of servers because a query may need to hop back and forth to retrieve all target data. 

Latency is critical for many graph workloads. 
In interactive workloads, where users send ad-hoc exploratory queries to the system, lower latency makes the system more usable and responsive. 
In longer-running queries, even relatively small latency slowdowns can add up easily, resulting in much larger running times and lower utilization.
Although some systems \cite{Wukong,Pragh,grasper} use advance hardware technologies such as Remote Direct Memory access to alleviate the network communication cost, inter-server traversal still significantly increase the performance of the system \cite{Pragh}. 
Various existing work \cite{MorphoSys,schism,SPAR} utilize data replication to mitigate the cost of inter-server traversals. 
However, their solutions propose algorithms to completely eliminate inter-server traversals, which introduces high replication costs.
Also, they do not provide the flexibility for users to decide the latency cost of queries. 
We argue that in reality, there exists a tradeoff between data replication and query latency. 
The more replicas we create, the fewer number inter-server hops a query requires, but at the same time, the higher the storage cost and synchronization cost the system will have. 
Existing work are on the latency extreme of the spectrum, and they fail to address the tradeoff between replication and latency. 

In this paper, we propose a tunable replication algorithm to provide users the flexibility to pick a point on the latency and replication spectrum. 
Instead of ensuring all queries will not require any server hops, we aim to generate a replication scheme such that a set of user-defined \emph{n}-hop queries will at most require \emph{k} server hops, where \emph{n} and \emph{k} are user-defined, and users can choose a suitable \emph{k} based on the latency requirement of that query and their replication budget. 

%We argue that, even though the problem has been investigated by previous work, existing solutions lead to excessive replication costs that make them impractical for graph workloads.
%Therefore, we cast the problem of data replication for graph workloads under a different perspective and show how this new problem definition opens up new research questions.
% \ms{We should mention somewhere that we focus on vertex partitioning and not edge partitioning. In edge partitioning  some vertices are already replicates initially. however, it's not com to use edge partitioning in graph dbs as far  as i can tell. }

\subsection{Motivating Experiment}
\nn{move to section 2?}
To show the remote access property of multi-hop queries and the limitations of existing work, we conduct a motivating experiment using the LDBC's Social Network Benchmark (LDBC SNB) \cite{ldbc}, which is currently the best-known benchmark for graph query workloads.
We generate a synthetic social network (30M vertices) with a power-law structure using the SNB data generator. 
We use the set of interactive short read queries in the SNB workload because they generally have lower latency, and inter-server traversal will be the bottleneck of the query.  
We generate a set of query parameters using the benchmark. 
We assume that the data are partitioned across a varying number of servers. 
We show the result of three partitioning scheme, namely \emph{hash partitioning}, \emph{graph partitioning}, and \emph{hypergraph partitioning}. 
\emph{Hash partitioning} uses a hash function to hash the vertex id to decide which server to store the vertex and is the most common data partitioning scheme adopted in practice because of its simplicity.  
For \emph{graph partitioning}, we use metis to partition the data graph into |servers| subgraphs while minimizing edge cuts. 
We store all vertices in each subgraph to the corresponding server. 
\emph{Hypergraph partitioning} is inspired by \cite{schism,social_hash}. 
It samples and models the workload into a hypergraph. A data vertex is represented as a node, and all data vertices accessed in a query are grouped into a hyperedge. 
We then use hmetis to partition the workload hypergraph into |servers| subgraphs and store the subgraphs into servers accordingly. 

We run the sample queries and plot the CDF of the number of hops in the longest path of the queries, shown in Figure \ref{fig:short_queries_remote_per_q}. 
%We also analyze the workload for GNN training and real-time inference. 
%We generate the GNN workload by querying the $n$-hop neighborhood of 100k random starting points, where we randomly query 10 (for training) and all (for real-time inference \nn{cite?}) neighbors at each hop. 
We observe that most of the queries require at least one server hop in their critical path.
Moreover, the overall distribution has a long tail, which indicates that a small number of queries need to perform a large number of server hops to retrieve the target data and thus increasing the tail latency of the system. 
%For GNN workload, more than 65\% of the GNN queries require at least one server hop in their critical path. 
These results validate that multi-hop queries consist of inter-server hops in practice. 




\subsection{Related Work}
\nn{skip this because we have a dedicated section at the end of the paper?}
There have been various attempts to alleviate the network burden of distributed queries by leveraging data replication.
Schism \cite{schism} is a workload-aware data partitioning algorithm that aims to minimize the number of distributed transactions.
It uses a set of offline workload traces to generate a data partitioning scheme and a replication scheme.
However, it does not provide the flexibility for users to bound the latency cost. 
SPAR \cite{SPAR} and MorphoSys \cite{MorphoSys} provide a \emph{guarantee} on the number of server hops each query requires. 
SPAR guarantees all the 1-hop queries will only need to access one server to retrieve required data by proposing replication policies. 
In this case, the inter-server communication cost is reduced to 0 (i.e., no distributed accesses). 
However, SPAR only provides a \emph{0}-hop guarantee for 1-hop queries, and the algorithm cannot be naturally extended to multi-hop queries, which is a key type of operation in practice. 
MorphoSys provides a \emph{0}-hop guarantee for all queries by altering its physical design before query execution. 
Nevertheless, MorphoSys optimizes for transactional workloads, which primarily consist of range scans.
It assumes that the read set and write set of a query are known before the actual query execution. 
This assumption does not hold for graph workloads, as the next hop of a query is decided based on the previous hop and will not be known until query execution time. 
Moreover, MorphoSys does not provide a flexible latency budget for different queries. 


\subsection{Our Contributions}
In this paper, we make the following contributions. 
\begin{itemize}
    \item XX
\end{itemize}


\end{comment}

==> sections/cascading_replication_problem-old.tex <==
\section{Greedy Latency-Bound Replication}
In this section, we show that a greedy approach to solving the latency-bound replication problem does not necessarily result in correct solutions.
We then propose sufficient correctness conditions.


% \subsection{old text}
% Our goal is to find a replicated data placement function that respects the latency and load balancing constraints while minimizing replication cost (see Eqn.~\ref{eqn:problem} and~\ref{eqn:latency-cost-repl}).
% As discussed previously, the algorithm assumes the system uses the proposed routing function and considers only upward replication functions.
% The optimizing process is done offline based on the query workload, the data graph, the system configuration, and the latency requirements.

% Materializing all matches in the query workload is generally infeasible because of their potentially huge number and the memory size required.
% To resolve this, we propose a generic \emph{iterative} replication approach that iteratively updates the replication function to optimize each path of matches. 
% This iterative approach can bound the memory requirement and the computational complexity by controlling the number of paths it considers at a time.

% Perhaps surprisingly, adding replicas may increase the latency cost of previously optimized paths, leading to latency violations.
% We present this problem as the \emph{iterative violation problem} and discuss under what conditions it may arise.
% Finally, we introduce a sufficient condition on the replicated data placement function $r$ for a path $p$, such that if the condition holds on $r$, $p$ must satisfy its latency constraint regardless of future replica additions to $r$.

\subsection{A Generic Greedy Algorithm}
The latency-bound replication problem considers a potentially huge number of causal access trees, which are provided as input to model the workload.
A simple greedy solution is to consider each path of each tree in isolation and add replicas so that the latency constraint of that path is not violated.
Ensuring no path of any causal access tree violates its latency constraint is sufficient to respect the latency constraint of the optimization problem.
However, as we will show, greedily adding replicas for each path in isolation does not necessarily lead to a globally correct solution.

A generic greedy replication algorithm is shown in Algorithm~\ref{algo:generic}.
It iterates over all root-to-leaf paths $p$ in the causal access trees of the workload.
Given a path $p$, the \textsc{update} function performs the following: it adds new replicas to extend the current replicated data placement function $r_{i-1}$ to $r_i$, such that all paths visited so far, including $p$, satisfy their latency constraint under $r_i$. 

This algorithm assumes that all causal access trees of a workload are provided as input.
Our implementations of the greedy algorithms enumerate paths directly from the dataset without materializing all trees.
We considered graph datasets and query types that can be modeled as graphs.
For each path in query graphs, we enumerate all possible matching of the path in the dataset.
We prune redundant query paths that exist in multiple query graphs and only enumerate each query path once.
For queries that have parameters, we consider all possible combinations of parameters that the query path can access. 
The running time of iterating over all query paths is practically feasible, as shown in our evaluation.

% Recall that a match corresponds to the set of vertices accessed when executing the query with a specific set of parameters. 
% Matches of a query may involve redundant paths if one set of parameters is contained by the other. 
% To avoid redundant computation, instead of iterating though paths of matches, the algorithm enumerates all root-to-leaf paths of queries in the workload.
% At each iteration, it returns a path $p_i$ in $G$ matching the a root-to-leaf query path and the corresponding latency constraint.
% Note that we omit parameters of the query path when we generate $p_i$, which equals to considering all possible combinations of parameters that the query path can access. 
% %By processing paths one-by-one, the algorithm also has minimal memory requirements.
% The running time of iterating over all query paths is practically feasible, as shown in our evaluation.

% Given a path $p$, the \textsc{update} function adds new replicas to extend the current replicated data placement function $r_{i-1}$ to $r_i$, such that $p$ satisfies its latency constraint under $r$. 
% We now discuss how to implement a correct \textsc{update} function, such that the latency costs of all previously optimized paths will not violate its corresponding constraint in future extensions of $r$.

%The algorithm guarantees that for each $i < j$ and for each vertex $v \in V$, it holds that $r_i(v) \subseteq r_j (v)$.

\setlength{\textfloatsep}{0.5em}
\begin{algorithm}[t]
    \input{algorithms/framework.tex}
\end{algorithm}
\vspace{-3mm}
\subsection{Incorrect Greedy Updates}
Developing a greedy algorithm in our framework boils down to writing an \textsc{update} function.
It turns out that implementing a correct \textsc{update} function is not straightforward.
Iteratively adding new replicas to reduce the latency of \emph{one path} may increase the latency of \emph{some other paths}.
We show why this is the case considering the example of a simple but incorrect greedy algorithm.

\spara{A na\"{i}ve algorithm}
Consider an intuitive, yet incorrect, implementation of the \textsc{update} function as shown in Algorithm~\ref{algo:naive}.
The algorithm first sets up the latency budget of the path to the latency constraint of the query, $t_Q$.
It then traverses each pair of consecutive vertices $(v_{p_i}, v_{p_{i+1}})$ from root to leaf of $p$, accessing the master copy of a vertex and consuming the latency budget if needed, until it depletes its budget and is no longer allowed to perform any distributed traversal.
After that, the algorithm replicates all subsequent vertices in $p$ to the server storing the master copy of the last vertex we have reached in the path.
Note that the resulting replicated data placement function is an upward replication function because 
all replicated vertices are accessed at the same server of its parent in $p$ (i.e., the location of accessing the last reached vertex in $p$). 
%all replication happens from a child vertex to its parent (i.e., last reached vertex in $p$).

The algorithm guarantees that the latency constraint of path $p$ is respected. 
The additional replicas created to optimize $p$, however, might result in violations of the latency constraint for some other path that was optimized previously.
We call this an \emph{iterative violation}, and we demonstrate the idea using the following example.

\setlength{\textfloatsep}{0.5em}
\begin{algorithm}[t!]
    \input{algorithms/naive.tex}    
\end{algorithm}

\spara{Example of iterative violation}
% and assume that $l(s_i,s_j)=1$ for all $i \neq j$.
Consider the data graph $G$ on the left of Figure~\ref{fig:cascading_example}.
Suppose we are executing the \textsc{update} function on the path $p_1 = \langle v_2, v_4, v_6, v_8 \rangle$ with a latency constraint of $1$.

Without replicas (i.e., $r_0$), processing $p_1$ requires 3 distributed traversals, which violates its latency constraint.
The \textsc{update} function of Algorithm~\ref{algo:naive} first examines the pair of vertices $(v_2, v_4)$.
As the two vertices are located on different servers, traversing from $v_2$ to $v_4$ has a latency cost of $1$, and it depletes the latency budget.
The algorithm then examines the next pair of vertices $(v_4, v_6)$.
As they are also located on different servers, allowing a distributed traversal from $v_4$ to $v_6$ will exceed the latency constraint of $p_1$.
Therefore, the algorithm extends $r_0$ to $r_1$ by replicating subsequent vertices $v_6$ and $v_8$ to $d(v_4) = s_2$.
Under $r_1$, $p_1$ accesses $v_2$ at $s_1$ and then perform a distributed traversal to $d(v_4) = s_2$ to access all subsequent vertices $\langle v_4, v_6, v_8 \rangle$, resulting in a latency cost of $1$.

We now show that when the algorithm later adds new replicas to extend $r_1$ to optimize some path $p_2$, those replicas may increase the latency cost of $p_1$.
Suppose $p_2 = \langle v_5, v_3, v_4 \rangle$ (see Figure~\ref{fig:cascading_example}).
The latency cost of $p_2$ under $r_1$ is $2$, and suppose its latency constraint is $1$.
The \textsc{update} function of Algorithm~\ref{algo:naive} depletes the latency budget to traverse from $v_5$ to $v_3$ and replicates the remaining vertex $v_4$ to $d(v_3) = s_1$.
The resulting replicated data placement function $r_2$ extending $r_1$ satisfies the latency constraint for $p_2$.

Although $r_2$ avoids latency violation of $p_2$, it induces a latency violation of $p_1$. 
Specifically, under $r_2$, $p_1$ first accesses $v_2$ at $s_1$.
After that, it accesses the new replica of $v_4$ locally at $s_1$, instead of accessing the master copy of $v_4$ at $s_2$ as under $r_1$. 
Next, since $v_6$ does not exist in $s_1$, $p_1$ is routed to $s_3$ to access the master copy of $v_6$ according to the thrifty routing function, and then similarly routed to $s_4$ to access $v_8$. 
The latency cost of $p_1$ under $r_2$ is now $2$, which leads to a latency violation. 
Such violation happens because the additional replica introduced in $r_2$ changes the location of accessing $v_4$ in $p_1$.
Formally, $a_{r_1}(v_4) = d(v_4) = s_2$ under $r_1$, and $a_{r_2}(v_4) = a_{r_2}(v_2) = s_1$ under $r_2$, where $C$ is the causal access tree including $p_1$.
%Accessing $v_4$ and $v_2$ at $s_1$ means missing the replicas of $v_6$ and $v_8$ at $s_2$, which were previously leveraged to respect the latency bound under $r_0$.

\begin{figure}[]
    \includegraphics[width=\linewidth]{figures/cascading_example.pdf}
    \vspace{-1.7\baselineskip}
    \caption{Example of iterative violation. Thrifty routing paths are represented as dashed arrows. Replicas are represented in solid colors and are shown as part of the data graphs for ease of explanation. Accesses of $p_1$ and $p_2$ are highlighted in pink and green, respectively. }
    \label{fig:cascading_example}
    %\vspace*{-1em}
\end{figure}

\vspace{-1em}
\subsection{Correctness Conditions for Updates}
In this subsection, we present two sufficient conditions for an \textsc{update} function to be correct and to avoid iterative violations when using thrifty routing.
% The previous subsection shows that adding new replicas to extend the replicated data placement function may cause an iterative violation, which is a potential problem for any iterative replication algorithms.
% A correct algorithm must ensure that the latency constraints of optimized paths are never violated regardless of the future addition of replicas.
First, we define a property on the \emph{replicated data placement function} for a given path, which we call \emph{robustness}, and show that it avoids iterative violations of that path, regardless of how replicas are added in future iterations.
%If \emph{each} $r_i$ generated by the \textsc{update} function is robust, then \emph{all paths} satisfy their latency constraint.
Next, we show a sufficient condition for \emph{workloads} to be \emph{safe}. 
In a safe workload, any \textsc{update} function that incrementally adds replicas will be correct.


\spara{Robust replicated data placements}
We start by defining an extension of a replicated data placement function, which is the result of applying the \textsc{update} function to optimize a path.

\begin{definition}[Extension of a replicated data placement function]
    Let $r$ be a replicated data placement function for a dataset $D$. 
    A replicated data placement function $r'$ is an extension of $r$ for some object $v' \in D$ if and only if:
    $$
        (|r'(v') \setminus r(v')| = 1) \wedge
        (\forall v \neq v' \in D, r'(v) = r(v))
    $$
    
\end{definition}

% Note that this definition of extension considers adding only one object replica.
% Any extension adding multiple replicas for multiple objects can be seen as a sequence of single-object single-replica extensions as defined previously.

Next, we define an auxiliary notion \emph{traversal subpath}.
%Recall that the latency cost is represented in terms of the number of distributed traversals among servers.
Recall that the function $h$ describes the latency of a path in a causal access tree (see Eqn.~\ref{eqn:latency-subpath-repl}).
The traversal subpath of a root-to-leaf path $p$ of a causal access tree for some value $i$ is the subpath of $p$ consisting of vertices that are accessed after making the $i$-th distributed traversal and before another distributed traversal is required.

\begin{definition}[Traversal subpath]
    Let $p:\langle v_{p_1}, v_{p_2}, ..., v_{p_n}\rangle$ be a root-to-leaf path of causal access tree $C$ of a query,
    $r$ a replicated data placement function, and $a_r$ a thrifty routing function.
    A traversal subpath $g_{p,r}^i$ of $p$ under $r$ for $i$ is a subpath $g_{p,r}^i = \langle v_{p_j}, ..., v_{p_k}\rangle$  of $p$ such that $h(g_{p,r}^i, a_r) = 0$ and:
    \begin{itemize}
        \item if $j > 1$, then it holds that $h(\langle v_{p_1}, \ldots, v_{p_{j-1}} \rangle, a_r) = i$ and $a_r(v_{p_{j-1}}) \neq a_r(v_{p_j})$, and
        \item if $k < n$, then it holds that $a_r(v_{p_k}) \neq a_r(v_{p_{k+1}})$.  
    \end{itemize}
\end{definition}

The latency cost of a path equals the largest index of its traversal subpaths.
For example, the path $p_1$ in Figure \ref{fig:cascading_example} has 3 traversal subpaths under $r_2$: $g_{p_1,r_2}^0 = \langle v_2, v_4 \rangle$, $g_{p_1,r_2}^1 = \langle v_6 \rangle$, and $g_{p_1,r_2}^2 = \langle v_8 \rangle$, and has a latency cost of 2. 

We now define robustness and formally prove that it is a sufficient condition for a replicated data placement function to avoid iterative violations of a given path when using thrifty routing. 

\begin{definition}[Robust replicated data placement function]
    Let $p = \langle v_{p_1}, v_{p_2}, ..., v_{p_n}\rangle$ be a root-to-leaf path of causal access tree $C$ of a query, and
    $r$ a replicated data placement function.
    The replicated data placement function $r$ is robust for $p$ if and only if for each traversal subpath $g_{p,r}^i = \langle v_{p_j}, ..., v_{p_k}\rangle$ of path $p$ under $r$ it holds: $$\forall x,y \in[j,k], x < y : d(v_{p_x}) \in r(v_{p_y})$$
\end{definition}

\begin{lemma} \label{lem:inductive-robust}
    Let $r$ be a robust replicated data placement function for $p$ and $r'$ be an extension of $r$ for one or more objects. It follows that $r'$ is robust for $p$.
\end{lemma}
\begin{proof}
    This directly follows from the fact that $r'$ only adds replicas to $r$, so it preserves the robustness condition of $r$.
\end{proof}
% We prove that the robustness property is sufficient for outputting a correct replicated data placement function.

\begin{theorem}\label{thm:robust-correct}
    Let $p$ be a root-to-leaf path in a causal access tree $C$ of a query $Q$, $r$ a replicated data placement function, $a_r$ a thrifty routing function, and $t_Q$ an upper bound on latency of $Q$. 
    If $r$ is robust for $p$ and $h(p,a_r) \leq t$, there exists no replicated data placement function $r'$ extending $r$ for one object such that $h(p,a_r) > t$ under $r'$. 
\end{theorem}
\begin{proof}
    Assume by contradiction that $r$ is robust for $p$ and there exists an $r'$ extending $r$ such that $h(p,a_{r'}) > t$.
    This implies that $h(p,a_r) < h(p,a_{r'})$, so $r'$ must change the routing of some object $v$ in $p$, i.e., $a_r(v) \neq a_{r'}(v)$.
    %Let $a_M$ be the proposed routing function under $r$ and $a'_M$ be the proposed routing function under $r'$.
    %It must hold that $h(p, a_M) > 0$, since otherwise all vertices in $p$ can be matched at the server that contains the master copy of the root vertex of $p$, and there cannot exists an extension $r'$ of $r$ that causes a violation.
    %Therefore, matching $p$ requires at least one hop, that is, one inter-server RPC call.
    Let $p = \langle v_{p_1}, v_{p_2}, ..., v_{p_n}\rangle$, $m$ be the smallest index such that $a_r(v_{p_m}) \neq a_{r'}(v_{p_m})$, and $g_{p,r}^i = \langle v_{p_j}, ..., v_{p_k}\rangle$ be the traversal subpath under $r$ including $v_{p_m}$.
    By definition of traversal subpath, $a_r(v_{p_{j-1}}) \neq a_r(v_{p_j})$, so $a_r$ routes the query to access $v_{p_j}$ to $s=d(v_{p_j})= a_r(v_{p_j})$.
    The query then accesses the remaining objects in $g_{p,r}^i$ at $s$ since $h(g_{p,r}^i, a_r) = 0$.
    

    We previously determined that $a_r(v_{p_m}) \neq a_{r'}(v_{p_m})$.
    Since the routing for $v_{p_m}$ changes under $r'$, then $r'$ must have added a new replica for $v_{p_m}$ compared to $r$ and $a_{r'}(v_{p_m})$ must route the query to that replica to access $v_{p_m}$.
    It follows from Def.~\ref{eqn:constrained} that the new replica is placed with the predecessor of $v_{p_m}$ in $p$, that is, $a_{r'}(v_{p_m}) = a_{r'}(v_{p_{m-1}})$.
    Since $r'$ only adds one object replica for $v_{p_m}$, it holds that $a_{r'}(v_{p_{m-1}})= a_r(v_{p_{m-1}}) $.

    We have so far established that $a_r(v_{p_m}) \neq a_{r'}(v_{p_m})$, $a_{r'}(v_{p_m}) = a_{r'}(v_{p_{m-1}})$, and $a_{r'}(v_{p_{m-1}}) = a_r(v_{p_{m-1}})$, so it follows that $a_r(v_{p_m}) \neq a_r(v_{p_{m-1}})$.
    The vertex $v_{p_m}$ is in $g_{p,r}^i$ by definition, so it follows from the definition of traversal subpath that $v_{p_m} = v_{p_j}$.

    It follows that $a_{r'}(v_{p_j}) = a_{r'}(v_{p_{j-1}})$, so the query accesses $v_{p_j}$ locally under $r'$, without a distributed traversal. 
    This saves one distributed traversal compared to $a_r$, which routes the query to $d(v_{p_j})$.
    It now takes $i-1$ distributed traversals to reach $v_{p_j}$ under $r'$, so $v_{p_j}$ is in $g^{i-1}_{p, r'}$.
    We argued previously that $m = j$ is the minimum index where $a_r$ and $a_{r'}$ differ, so to increase the latency of $p$, $a_{r'}$ must perform at least two extra distributed traversals in $p$ after $v_{p_j}$.

    Let $v_{p_x}$ be the first object in $p$ after $v_{p_j}$ that causes a distributed traversal under $r'$, that is, such that $a_{r'}(v_{p_x}) \neq a_{r'}(v_{p_{x-1}})$.
    By definition, both $v_{p_j}$ and $v_{p_{x-1}}$ are in $g^{i-1}_{p, r'}$ under $r'$. 

    It follows from Def.~\ref{eqn:constrained} that $a_{r'}(v_{p_x}) = d(v_{p_x})$, so $a_{r'}$ routes the query to the master of $v_{p_x}$.
    We have shown that $v_{p_{x-1}}$ is in $g^{i-1}_{p, r'}$, so it takes $i-1$ distributed traversals to reach $v_{p_{x-1}}$ under $r'$ and one more distributed traversal to reach $v_{p_x}$, that is, $v_{p_x}$ is in $g^i_{p, r'}$.

    Let $g_{p,r}^o$ be the traversal subpath including $v_{p_x}$ under $r$.
    By definition of $g_{p,r}^o$, reaching $v_{p_x}$ requires $o$ distributed traversals under $r$.
    Since $x > j$ and $v_{p_j}$ is in $g_{p,r}^i$, it holds that $o \geq i$.
    Therefore, reaching $v_{p_x}$ under $r'$ does not require extra distributed traversals compared to $r$.

    We now show that there are no additional distributed traversals under $r'$ until we reach the last vertex in $g_{p,r}^o$. 
    Since $r$ is robust for $p$, it follows that for each object $v_{p_y}$ following $v_{p_x}$ in $g_p^o$, it holds that $d(v_{p_x}) \in r(v_{p_y})$.
    The same holds under $r'$ since $r'$ is also robust for $p$ according to Lemma~\ref{lem:inductive-robust}.
    This means that a local copy of each $v_{p_y}$ is available at $d(v_{p_x})$ so $a_{r'}(v_{p_y})=a_{r'}(v_{p_x})$.
    Therefore, matching the remaining objects in $g_{p,r}^o$ does not require distributed traversals.

    %We have shown that matching all objects until the end of $g_{p,r}^o$ does not require additional distributed traversals in $r'$ compared to $r$.
    In summary, so far we first proved that $r'$ does not introduce additional distributed traversals compared to $r$ to access $v_{p_j}$.
    Then, we showed that if $v_{p_x}$ is the first element after $v_{p_j}$ in $p$ that causes a distributed traversal in $r'$, accessing $v_{p_x}$ or any object in its subpath does not cause additional distributed traversals compared to $r$. 
    The same argument can be applied inductively for the next object in $p$ that requires a distributed traversal under $r'$ after $v_{p_x}$, if it exists.
    Therefore, $r'$ does not require extra distributed traversals compared to $r$ so $h(p,a_{r'}) \leq h(p,a_r) < t$, a contradiction. 
\end{proof}

The claim of Theorem~\ref{thm:robust-correct} also holds if $r'$ extends $r$ for multiple objects.
This can be proven inductively by extending $r$ for a single object at a time and by applying Theorem~\ref{thm:robust-correct} and Lemma~\ref{lem:inductive-robust} for each extension.
Therefore, we can conclude the following correctness condition on the output of the \textsc{update} function.

\begin{corollary}
    The replicated data placement function returned by Algorithm~\ref{algo:generic} respects the latency constraints on all paths of all causal access trees of all queries in $W$ if, for each value of $i$, $r_i$ respects the latency constraint on $p_i$ and is robust for $p_i$.
\end{corollary}

\spara{Safe workloads}
We define a class of workloads for which any \textsc{update} function is correct, regardless of the robustness of its output.

\begin{definition}[Safe workload]
    A workload $W$ is safe when using the thrifty routing function if and only if for every causal access tree $C$ of every query $Q \in W$, it holds that the height of $C$ is $n$ and $t_Q \in \{0, n-1, n\}$, where $t_Q$ is the latency constraint of query $Q$. 
    
\end{definition}

\begin{theorem}
    Let $D$ be a dataset, $W$ be a workload, $S$ be a set of servers, and $r$ a replicated data placement function over $D$ and $S$ such that for each $Q \in W$ it holds $l_Q \leq t_Q$ under $r$, where $t_Q$ is the latency constraint for $Q$.
    If $W$ is safe, there exists no replicated data placement function $r'$ extending $r$ for some object $v' \in D$ such that $l_Q > t_Q$ under $r'$ for some query $Q \in W$. 
    \label{theorem:hop_bound}
\end{theorem}
\begin{proof}
    Assume by contradiction that $W$ is safe and there exist an $r'$ extending $r$ for $v$ such that $l_Q > t_Q$ under $r'$.
    By the definition of safe, we know that $t_Q \in \{0, n-1, n\}$.
    We first prove the case $t_Q=0$.
    Since $l_Q \leq t_Q = 0$ under $r$ by hypothesis, the query is always routed to the master of the root vertex, and all vertices in each causal access tree $C$ of $Q$ must be replicated in the same server. 
    The function $r'$ adds a new replica to $r$ cannot change the routing $a_r$, which is defined by Def.~\ref{eqn:constrained}.
    Therefore, the latency of the query is still $0$ under $r'$, a contradiction.

    The case $t_Q = n$ is trivial: as the height of $C$ is $n$, the upper bound of $l_Q$ under any replicated data placement function is $n$, so $t_Q$ cannot be violated.

    Finally, we consider the case $t_Q = n-1$. 
    If $r'$ changes the latency $l_Q$ compared to $r$, it must change the routing for causal access tree $C$.
    According to Def.~\ref{eqn:constrained}, this can only happen if a replica of an object in $C$ is placed together with its predecessor in a root-to-leaf path of $C$.
    As mentioned in the previous case, the upper bound of $l_Q$ is $n$.
    Modifying the routing means at least one object can be accessed at the same server as its predecessor.
    The upper bound on $l_Q$ becomes $n-1$, which is not larger than $t_Q$, a contradiction.
\end{proof}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/local_min_example.pdf}
    \vspace{-1\baselineskip}
    \caption{Example causal access trees. Co-optimized paths are highlighted in red. } 
    \label{fig:short_q_7}
    %\vspace{-1em}
\end{figure}


\begin{comment}
\spara{Making incremental updates robust}
To show how to enforce the robustness condition, we integrate it in the naive replication algorithm of Algorithm~\ref{algo:naive} and present the robust version in Algorithm~\ref{algo:cascading_proof}. 

\begin{algorithm}[t]
\input{algorithms/naive-robust.tex}
\end{algorithm}

We traverse each pair of vertices $v_i, v_{i+1}$ from root to leaf of $p$ and consume the latency budget if needed. 
In addition, at each step from $v_i$ to $v_{i+1}$, we record the \emph{index} of the first vertex of the current $i$-hop subpath.
Like in the previous algorithm, when the budget is depleted, we replicate the remaining vertices in $p$ to the last server $d(v_{p_i})$ the query accesses. 
Additionally, to ensure that robustness holds for the current $i$-hop subpath, we replicate each vertex $v_j$ in the $i$-hop subpath to all the master server of its preceding vertices in the subpath. 
No additional replicas are required to make robustness hold for the subsequent $j$-hop subpaths with $j>i$.
\end{comment}

==> sections/cascading_replication_problem.tex <==
\section{Greedy Heuristics}
In this section, we show that a greedy approach to solving the latency-bound replication problem does not necessarily result in correct solutions.
We then propose sufficient correctness conditions.


% \subsection{old text}
% Our goal is to find a replicated data placement function that respects the latency and load balancing constraints while minimizing replication cost (see Eqn.~\ref{eqn:problem} and~\ref{eqn:latency-cost-repl}).
% As discussed previously, the algorithm assumes the system uses the proposed routing function and considers only upward replication functions.
% The optimizing process is done offline based on the query workload, the data graph, the system configuration, and the latency requirements.

% Materializing all matches in the query workload is generally infeasible because of their potentially huge number and the memory size required.
% To resolve this, we propose a generic \emph{iterative} replication approach that iteratively updates the replication function to optimize each path of matches. 
% This iterative approach can bound the memory requirement and the computational complexity by controlling the number of paths it considers at a time.

% Perhaps surprisingly, adding replicas may increase the latency cost of previously optimized paths, leading to latency violations.
% We present this problem as the \emph{iterative violation problem} and discuss under what conditions it may arise.
% Finally, we introduce a sufficient condition on the replicated data placement function $r$ for a path $p$, such that if the condition holds on $r$, $p$ must satisfy its latency constraint regardless of future replica additions to $r$.

\subsection{A Generic Greedy Algorithm}
The latency-bound replication problem considers a potentially huge number of causal access trees, which are provided as input to model the workload.
A simple greedy solution is to consider each path of each tree in isolation and add replicas so that the latency constraint of that path is not violated.
Ensuring no path of any causal access tree violates its latency constraint is sufficient to respect the latency constraint of the optimization problem.
However, as we will show, greedily adding replicas for each path in isolation does not necessarily lead to a globally correct solution.

A generic greedy replication algorithm is shown in Algorithm~\ref{algo:generic}.
It iterates over all root-to-leaf paths $p$ in the causal access trees of the workload.
Given a path $p$, the \textsc{update} function performs the following: it adds new replicas to extend the current replicated data placement function $r_{i-1}$ to $r_i$, such that all paths visited so far, including $p$, satisfy their latency constraint under $r_i$. 

This algorithm assumes that all causal access trees of a workload are provided as input.
Our implementations of the greedy algorithms enumerate paths directly from the dataset without materializing all trees.
We considered graph datasets and query types that can be modeled as graphs.
For each path in query graphs, we enumerate all possible matching of the path in the dataset.
We prune redundant query paths that exist in multiple query graphs and only enumerate each query path once.
For queries that have parameters, we consider all possible combinations of parameters that the query path can access. 
The running time of iterating over all query paths is practically feasible, as shown in our evaluation.

% Recall that a match corresponds to the set of vertices accessed when executing the query with a specific set of parameters. 
% Matches of a query may involve redundant paths if one set of parameters is contained by the other. 
% To avoid redundant computation, instead of iterating though paths of matches, the algorithm enumerates all root-to-leaf paths of queries in the workload.
% At each iteration, it returns a path $p_i$ in $G$ matching the a root-to-leaf query path and the corresponding latency constraint.
% Note that we omit parameters of the query path when we generate $p_i$, which equals to considering all possible combinations of parameters that the query path can access. 
% %By processing paths one-by-one, the algorithm also has minimal memory requirements.
% The running time of iterating over all query paths is practically feasible, as shown in our evaluation.

% Given a path $p$, the \textsc{update} function adds new replicas to extend the current replicated data placement function $r_{i-1}$ to $r_i$, such that $p$ satisfies its latency constraint under $r$. 
% We now discuss how to implement a correct \textsc{update} function, such that the latency costs of all previously optimized paths will not violate its corresponding constraint in future extensions of $r$.

%The algorithm guarantees that for each $i < j$ and for each vertex $v \in V$, it holds that $r_i(v) \subseteq r_j (v)$.

\setlength{\textfloatsep}{0.5em}
\begin{algorithm}[t]
    \input{algorithms/framework.tex}
\end{algorithm}
\vspace{-3mm}


\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/upward_downward_G.pdf}
        \caption{Dataset graph.}
        \label{fig:up_down_G}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.31\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/downward_replication.pdf}
        \caption{Routing with arbitrary replication.}
        \label{fig:downward_replication}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/upward_replication.pdf}
        \caption{Thrifty routing + upward replication.}
        \label{fig:upward_replication}
    \end{subfigure}
        \vspace{-0.5\baselineskip}
       \caption{Examples of possible routing paths under different replication decisions. Replicas are represented in solid colors. Routing paths are represented as dashed arrows. }
       \label{fig:upward_downward_replication}
\end{figure}

\subsection{Pruning the Search Space}
This restricts the search space for solutions to the problem, we describe a class of functions, namely \emph{upward replication functions}, that includes all optimal solutions to the latency-bound replication problem when using thrifty routing.
Implementations of the \textsc{UPDATE} function can then only explore upward replication functions as candidate solutions.

\begin{definition}[Upward replication function]
    Let $D$ be a dataset and $W = \{ Q_1, \ldots, Q_m\}$ be a workload consisting of a set of queries.
    A replicated data placement function $r$ is an upward replication function if the following holds: $a(r,v) \neq d(v)$ for some causal access tree $C$ of a query $Q_i\in W$ in $G$ and non-root node $v$ of $C$ implies that $a(r,u) = a(r,v)$ for the parent $u$ of $v$ in $C$.
    \label{def:upward_replication}
\end{definition}

An example of an upward replication function is shown in Figure~\ref{fig:upward_replication}.
%Given a root-to-leaf path $p$ of a causal access tree, Upward replication updates only replicate child vertices to the server of their parent vertex in $p$. 
Replicating $v_6$ onto $s_2$ satisfy the definition because when matching $\langle v_2, v_4, v_6\rangle$, the query executor accesses $v_4$ at $s_2$ before $v_6$.
 %replicating $v_6$ to the server of its parent node $v_4$'s server $s_2$, and replicating $v_4$ to its parent server $s_1$ are considered as upward replication updates. 

We prove that any optimal solution to the latency-bound replication problem must be an upward replication function. 

\begin{theorem}
    In a system using thrifty routing, any optimal replicated data placement function solving the latency-bound replication problem is an upward replication function. 
\end{theorem}
\begin{proof}
    If an optimal replicated data placement function $r$ contains no additional object replicas compared to $d$, the proof follows directly from Def.~\ref{def:upward_replication}.
    If not, a replicated data placement function $r$ is optimal according to  Eqn.~\ref{eqn:problem} if and only if removing any object replica increases the latency of some query.
    This implies that each object replica must be accessed in some causal access tree.
    Formally, for each replicated object $v \in D$ and for each location of the replica $s \in r(v) \setminus \{d(v)\} $, 
    there must exist some causal access tree $C'$ of a query $Q\in W$ such that $a(r,u) = s$ for the parent $u$ of $v$ in $C'$.
    %there must be a parent $u$ of $v$ in some causal access tree $C'$ of a query $Q\in W$ such that $a(r,u) = s$ .
    
    Let $v$ be a replicated object in $D$ and $s$ be one of the servers where it is replicated.
    Assume that the system uses a thrifty routing function.
    We now show that any optimal replicated data placement function $r$ is an upward replication function, which according to Def.~\ref{def:upward_replication} implies that there exists some causal access tree $C$ such that $a(r,u) = a(r,v) = s$ for the parent $u$ of $v$ in $C$.
    
    Assume by contradiction that there exists no such $u$ for some replicated object $v \in D$.
    This means that for all causal access tree $C$ that accesses the replicated object $v$, if $a(r,v) = s$, $a(r,u) \neq a(r,v)$ for the parent $u$ of $v$ in $C$.
    By hypothesis, $a_r$ is a thrifty routing function.
    According to Def.~\ref{eqn:constrained}, if $a(r,u) \neq a(r,v)$, then $a(r,v) = d(v)$, and this holds for all causal access trees $C$ that includes $v$.
    However, this contradicts our previous finding that $a(r,v) = s \neq d(v)$ for some causal access tree $C'$.
\end{proof}

\subsection{Incorrect Greedy Updates}
Developing a greedy algorithm in our framework boils down to writing an \textsc{update} function.
It turns out that implementing a correct \textsc{update} function is not straightforward.
Iteratively adding new replicas to reduce the latency of \emph{one path} may increase the latency of \emph{some other paths}.
We show why this is the case considering the example of a simple but incorrect greedy algorithm.

\spara{A na\"{i}ve algorithm}
Consider an intuitive, yet incorrect, implementation of the \textsc{update} function as shown in Algorithm~\ref{algo:naive}.
The algorithm first sets up the latency budget of the path to the latency constraint of the query, $t_Q$.
It then traverses each pair of consecutive vertices $(v_{p_i}, v_{p_{i+1}})$ from root to leaf of $p$, accessing the master copy of a vertex and consuming the latency budget if needed, until it depletes its budget and is no longer allowed to perform any distributed traversal.
After that, the algorithm replicates all subsequent vertices in $p$ to the server storing the master copy of the last vertex we have reached in the path.
Note that the resulting replicated data placement function is an upward replication function because 
all replicated vertices are accessed at the same server of its parent in $p$ (i.e., the location of accessing the last reached vertex in $p$). 
%all replication happens from a child vertex to its parent (i.e., last reached vertex in $p$).

The algorithm guarantees that the latency constraint of path $p$ is respected. 
The additional replicas created to optimize $p$, however, might result in violations of the latency constraint for some other path that was optimized previously.
We call this an \emph{iterative violation}, and we demonstrate the idea using the following example.

\setlength{\textfloatsep}{0.5em}
\begin{algorithm}[t!]
    \input{algorithms/naive.tex}    
\end{algorithm}

\spara{Example of iterative violation}
% and assume that $l(s_i,s_j)=1$ for all $i \neq j$.
Consider the data graph $G$ on the left of Figure~\ref{fig:cascading_example}.
Suppose we are executing the \textsc{update} function on the path $p_1 = \langle v_2, v_4, v_6, v_8 \rangle$ with a latency constraint of $1$.

Without replicas (i.e., $r_0$), processing $p_1$ requires 3 distributed traversals, which violates its latency constraint.
The \textsc{update} function of Algorithm~\ref{algo:naive} first examines the pair of vertices $(v_2, v_4)$.
As the two vertices are located on different servers, traversing from $v_2$ to $v_4$ has a latency cost of $1$, and it depletes the latency budget.
The algorithm then examines the next pair of vertices $(v_4, v_6)$.
As they are also located on different servers, allowing a distributed traversal from $v_4$ to $v_6$ will exceed the latency constraint of $p_1$.
Therefore, the algorithm extends $r_0$ to $r_1$ by replicating subsequent vertices $v_6$ and $v_8$ to $d(v_4) = s_2$.
Under $r_1$, $p_1$ accesses $v_2$ at $s_1$ and then perform a distributed traversal to $d(v_4) = s_2$ to access all subsequent vertices $\langle v_4, v_6, v_8 \rangle$, resulting in a latency cost of $1$.

We now show that when the algorithm later adds new replicas to extend $r_1$ to optimize some path $p_2$, those replicas may increase the latency cost of $p_1$.
Suppose $p_2 = \langle v_5, v_3, v_4 \rangle$ (see Figure~\ref{fig:cascading_example}).
The latency cost of $p_2$ under $r_1$ is $2$, and suppose its latency constraint is $1$.
The \textsc{update} function of Algorithm~\ref{algo:naive} depletes the latency budget to traverse from $v_5$ to $v_3$ and replicates the remaining vertex $v_4$ to $d(v_3) = s_1$.
The resulting replicated data placement function $r_2$ extending $r_1$ satisfies the latency constraint for $p_2$.

Although $r_2$ avoids latency violation of $p_2$, it induces a latency violation of $p_1$. 
Specifically, under $r_2$, $p_1$ first accesses $v_2$ at $s_1$.
After that, it accesses the new replica of $v_4$ locally at $s_1$, instead of accessing the master copy of $v_4$ at $s_2$ as under $r_1$. 
Next, since $v_6$ does not exist in $s_1$, $p_1$ is routed to $s_3$ to access the master copy of $v_6$ according to the thrifty routing function, and then similarly routed to $s_4$ to access $v_8$. 
The latency cost of $p_1$ under $r_2$ is now $2$, which leads to a latency violation. 
Such violation happens because the additional replica introduced in $r_2$ changes the location of accessing $v_4$ in $p_1$.
Formally, $a_{r_1}(v_4) = d(v_4) = s_2$ under $r_1$, and $a_{r_2}(v_4) = a_{r_2}(v_2) = s_1$ under $r_2$, where $C$ is the causal access tree including $p_1$.
%Accessing $v_4$ and $v_2$ at $s_1$ means missing the replicas of $v_6$ and $v_8$ at $s_2$, which were previously leveraged to respect the latency bound under $r_0$.

\begin{figure}[]
    \includegraphics[width=\linewidth]{figures/cascading_example.pdf}
    \vspace{-1.7\baselineskip}
    \caption{Example of iterative violation. Thrifty routing paths are represented as dashed arrows. Replicas are represented in solid colors and are shown as part of the data graphs for ease of explanation. Accesses of $p_1$ and $p_2$ are highlighted in pink and green, respectively. }
    \label{fig:cascading_example}
    %\vspace*{-1em}
\end{figure}

\vspace{-1em}
\subsection{Correctness Conditions for Updates}
In this subsection, we present two sufficient conditions for an \textsc{update} function to be correct and to avoid iterative violations when using thrifty routing.
% The previous subsection shows that adding new replicas to extend the replicated data placement function may cause an iterative violation, which is a potential problem for any iterative replication algorithms.
% A correct algorithm must ensure that the latency constraints of optimized paths are never violated regardless of the future addition of replicas.
First, we define a property on the \emph{replicated data placement function} for a given path, which we call \emph{robustness}, and show that it avoids iterative violations of that path, regardless of how replicas are added in future iterations.
%If \emph{each} $r_i$ generated by the \textsc{update} function is robust, then \emph{all paths} satisfy their latency constraint.
Next, we show a sufficient condition for \emph{workloads} to be \emph{safe}. 
In a safe workload, any \textsc{update} function that incrementally adds replicas will be correct.


\spara{Robust replicated data placements}
We start by defining an extension of a replicated data placement function, which is the result of applying the \textsc{update} function to optimize a path.

\begin{definition}[Extension of a replicated data placement function]
    Let $r$ be a replicated data placement function for a dataset $D$. 
    A replicated data placement function $r'$ is an extension of $r$ for some object $v' \in D$ if and only if:
    $$
        (|r'(v') \setminus r(v')| = 1) \wedge
        (\forall v \neq v' \in D, r'(v) = r(v))
    $$
    
\end{definition}

% Note that this definition of extension considers adding only one object replica.
% Any extension adding multiple replicas for multiple objects can be seen as a sequence of single-object single-replica extensions as defined previously.

Next, we define an auxiliary notion \emph{traversal subpath}.
%Recall that the latency cost is represented in terms of the number of distributed traversals among servers.
Recall that the function $h$ describes the latency of a path in a causal access tree (see Eqn.~\ref{eqn:latency-subpath-repl}).
The traversal subpath of a root-to-leaf path $p$ of a causal access tree for some value $i$ is the subpath of $p$ consisting of vertices that are accessed after making the $i$-th distributed traversal and before another distributed traversal is required.

\begin{definition}[Traversal subpath]
    Let $p:\langle v_{p_1}, v_{p_2}, ..., v_{p_n}\rangle$ be a root-to-leaf path of causal access tree $C$ of a query,
    $r$ a replicated data placement function, and $a_r$ a thrifty routing function.
    A traversal subpath $g_{p,r}^i$ of $p$ under $r$ for $i$ is a subpath $g_{p,r}^i = \langle v_{p_j}, ..., v_{p_k}\rangle$  of $p$ such that $h(g_{p,r}^i, a_r) = 0$ and:
    \begin{itemize}
        \item if $j > 1$, then it holds that $h(\langle v_{p_1}, \ldots, v_{p_{j-1}} \rangle, a_r) = i$ and $a(r,v_{p_{j-1}}) \neq a(r,v_{p_j})$, and
        \item if $k < n$, then it holds that $a(r,v_{p_k}) \neq a(r,v_{p_{k+1}})$.  
    \end{itemize}
\end{definition}

The latency cost of a path equals the largest index of its traversal subpaths.
For example, the path $p_1$ in Figure \ref{fig:cascading_example} has 3 traversal subpaths under $r_2$: $g_{p_1,r_2}^0 = \langle v_2, v_4 \rangle$, $g_{p_1,r_2}^1 = \langle v_6 \rangle$, and $g_{p_1,r_2}^2 = \langle v_8 \rangle$, and has a latency cost of 2. 

We now define robustness and formally prove that it is a sufficient condition for a replicated data placement function to avoid iterative violations of a given path when using thrifty routing. 

\begin{definition}[Robust replicated data placement function]
    Let $p = \langle v_{p_1}, v_{p_2}, ..., v_{p_n}\rangle$ be a root-to-leaf path of causal access tree $C$ of a query, and
    $r$ a replicated data placement function.
    The replicated data placement function $r$ is robust for $p$ if and only if for each traversal subpath $g_{p,r}^i = \langle v_{p_j}, ..., v_{p_k}\rangle$ of path $p$ under $r$ it holds: $$\forall x,y \in[j,k], x < y : d(v_{p_x}) \in r(v_{p_y})$$
\end{definition}

\begin{lemma} \label{lem:inductive-robust}
    Let $r$ be a robust replicated data placement function for $p$ and $r'$ be an extension of $r$ for one or more objects. It follows that $r'$ is robust for $p$.
\end{lemma}
\begin{proof}
    This directly follows from the fact that $r'$ only adds replicas to $r$, so it preserves the robustness condition of $r$.
\end{proof}
% We prove that the robustness property is sufficient for outputting a correct replicated data placement function.

\begin{theorem}\label{thm:robust-correct}
    Let $p$ be a root-to-leaf path in a causal access tree $C$ of a query $Q$, $r$ a replicated data placement function, $a_r$ a thrifty routing function, and $t_Q$ an upper bound on latency of $Q$. 
    If $r$ is robust for $p$ and $h(p,a_r) \leq t$, there exists no replicated data placement function $r'$ extending $r$ for one object such that $h(p,a_r) > t$ under $r'$. 
\end{theorem}
\begin{proof}
    Assume by contradiction that $r$ is robust for $p$ and there exists an $r'$ extending $r$ such that $h(p,a_{r'}) > t$.
    This implies that $h(p,a_r) < h(p,a_{r'})$, so $r'$ must change the routing of some object $v$ in $p$, i.e., $a(r,v) \neq a_{r'}(v)$.
    %Let $a_M$ be the proposed routing function under $r$ and $a'_M$ be the proposed routing function under $r'$.
    %It must hold that $h(p, a_M) > 0$, since otherwise all vertices in $p$ can be matched at the server that contains the master copy of the root vertex of $p$, and there cannot exists an extension $r'$ of $r$ that causes a violation.
    %Therefore, matching $p$ requires at least one hop, that is, one inter-server RPC call.
    Let $p = \langle v_{p_1}, v_{p_2}, ..., v_{p_n}\rangle$, $m$ be the smallest index such that $a(r,v_{p_m}) \neq a_{r'}(v_{p_m})$, and $g_{p,r}^i = \langle v_{p_j}, ..., v_{p_k}\rangle$ be the traversal subpath under $r$ including $v_{p_m}$.
    By definition of traversal subpath, $a(r,v_{p_{j-1}}) \neq a(r,v_{p_j})$, so $a_r$ routes the query to access $v_{p_j}$ to $s=d(v_{p_j})= a(r,v_{p_j})$.
    The query then accesses the remaining objects in $g_{p,r}^i$ at $s$ since $h(g_{p,r}^i, a_r) = 0$.
    

    We previously determined that $a(r,v_{p_m}) \neq a_{r'}(v_{p_m})$.
    Since the routing for $v_{p_m}$ changes under $r'$, then $r'$ must have added a new replica for $v_{p_m}$ compared to $r$ and $a_{r'}(v_{p_m})$ must route the query to that replica to access $v_{p_m}$.
    It follows from Def.~\ref{eqn:constrained} that the new replica is placed with the predecessor of $v_{p_m}$ in $p$, that is, $a_{r'}(v_{p_m}) = a_{r'}(v_{p_{m-1}})$.
    Since $r'$ only adds one object replica for $v_{p_m}$, it holds that $a_{r'}(v_{p_{m-1}})= a(r,v_{p_{m-1}}) $.

    We have so far established that $a(r,v_{p_m}) \neq a_{r'}(v_{p_m})$, $a_{r'}(v_{p_m}) = a_{r'}(v_{p_{m-1}})$, and $a_{r'}(v_{p_{m-1}}) = a(r,v_{p_{m-1}})$, so it follows that $a(r,v_{p_m}) \neq a(r,v_{p_{m-1}})$.
    The vertex $v_{p_m}$ is in $g_{p,r}^i$ by definition, so it follows from the definition of traversal subpath that $v_{p_m} = v_{p_j}$.

    It follows that $a_{r'}(v_{p_j}) = a_{r'}(v_{p_{j-1}})$, so the query accesses $v_{p_j}$ locally under $r'$, without a distributed traversal. 
    This saves one distributed traversal compared to $a_r$, which routes the query to $d(v_{p_j})$.
    It now takes $i-1$ distributed traversals to reach $v_{p_j}$ under $r'$, so $v_{p_j}$ is in $g^{i-1}_{p, r'}$.
    We argued previously that $m = j$ is the minimum index where $a_r$ and $a_{r'}$ differ, so to increase the latency of $p$, $a_{r'}$ must perform at least two extra distributed traversals in $p$ after $v_{p_j}$.

    Let $v_{p_x}$ be the first object in $p$ after $v_{p_j}$ that causes a distributed traversal under $r'$, that is, such that $a_{r'}(v_{p_x}) \neq a_{r'}(v_{p_{x-1}})$.
    By definition, both $v_{p_j}$ and $v_{p_{x-1}}$ are in $g^{i-1}_{p, r'}$ under $r'$. 

    It follows from Def.~\ref{eqn:constrained} that $a_{r'}(v_{p_x}) = d(v_{p_x})$, so $a_{r'}$ routes the query to the master of $v_{p_x}$.
    We have shown that $v_{p_{x-1}}$ is in $g^{i-1}_{p, r'}$, so it takes $i-1$ distributed traversals to reach $v_{p_{x-1}}$ under $r'$ and one more distributed traversal to reach $v_{p_x}$, that is, $v_{p_x}$ is in $g^i_{p, r'}$.

    Let $g_{p,r}^o$ be the traversal subpath including $v_{p_x}$ under $r$.
    By definition of $g_{p,r}^o$, reaching $v_{p_x}$ requires $o$ distributed traversals under $r$.
    Since $x > j$ and $v_{p_j}$ is in $g_{p,r}^i$, it holds that $o \geq i$.
    Therefore, reaching $v_{p_x}$ under $r'$ does not require extra distributed traversals compared to $r$.

    We now show that there are no additional distributed traversals under $r'$ until we reach the last vertex in $g_{p,r}^o$. 
    Since $r$ is robust for $p$, it follows that for each object $v_{p_y}$ following $v_{p_x}$ in $g_p^o$, it holds that $d(v_{p_x}) \in r(v_{p_y})$.
    The same holds under $r'$ since $r'$ is also robust for $p$ according to Lemma~\ref{lem:inductive-robust}.
    This means that a local copy of each $v_{p_y}$ is available at $d(v_{p_x})$ so $a_{r'}(v_{p_y})=a_{r'}(v_{p_x})$.
    Therefore, matching the remaining objects in $g_{p,r}^o$ does not require distributed traversals.

    %We have shown that matching all objects until the end of $g_{p,r}^o$ does not require additional distributed traversals in $r'$ compared to $r$.
    In summary, so far we first proved that $r'$ does not introduce additional distributed traversals compared to $r$ to access $v_{p_j}$.
    Then, we showed that if $v_{p_x}$ is the first element after $v_{p_j}$ in $p$ that causes a distributed traversal in $r'$, accessing $v_{p_x}$ or any object in its subpath does not cause additional distributed traversals compared to $r$. 
    The same argument can be applied inductively for the next object in $p$ that requires a distributed traversal under $r'$ after $v_{p_x}$, if it exists.
    Therefore, $r'$ does not require extra distributed traversals compared to $r$ so $h(p,a_{r'}) \leq h(p,a_r) < t$, a contradiction. 
\end{proof}

The claim of Theorem~\ref{thm:robust-correct} also holds if $r'$ extends $r$ for multiple objects.
This can be proven inductively by extending $r$ for a single object at a time and by applying Theorem~\ref{thm:robust-correct} and Lemma~\ref{lem:inductive-robust} for each extension.
Therefore, we can conclude the following correctness condition on the output of the \textsc{update} function.

\begin{corollary}
    The replicated data placement function returned by Algorithm~\ref{algo:generic} respects the latency constraints on all paths of all causal access trees of all queries in $W$ if, for each value of $i$, $r_i$ respects the latency constraint on $p_i$ and is robust for $p_i$.
\end{corollary}

\spara{Safe workloads}
We define a class of workloads for which any \textsc{update} function is correct, regardless of the robustness of its output.

\begin{definition}[Safe workload]
    A workload $W$ is safe when using the thrifty routing function if and only if for every causal access tree $C$ of every query $Q \in W$, it holds that the height of $C$ is $n$ and $t_Q \in \{0, n-1, n\}$, where $t_Q$ is the latency constraint of query $Q$. 
    
\end{definition}

\begin{theorem}
    Let $D$ be a dataset, $W$ be a workload, $S$ be a set of servers, and $r$ a replicated data placement function over $D$ and $S$ such that for each $Q \in W$ it holds $l_Q \leq t_Q$ under $r$, where $t_Q$ is the latency constraint for $Q$.
    If $W$ is safe, there exists no replicated data placement function $r'$ extending $r$ for some object $v' \in D$ such that $l_Q > t_Q$ under $r'$ for some query $Q \in W$. 
    \label{theorem:hop_bound}
\end{theorem}
\begin{proof}
    Assume by contradiction that $W$ is safe and there exist an $r'$ extending $r$ for $v$ such that $l_Q > t_Q$ under $r'$.
    By the definition of safe, we know that $t_Q \in \{0, n-1, n\}$.
    We first prove the case $t_Q=0$.
    Since $l_Q \leq t_Q = 0$ under $r$ by hypothesis, the query is always routed to the master of the root vertex, and all vertices in each causal access tree $C$ of $Q$ must be replicated in the same server. 
    The function $r'$ adds a new replica to $r$ cannot change the routing $a_r$, which is defined by Def.~\ref{eqn:constrained}.
    Therefore, the latency of the query is still $0$ under $r'$, a contradiction.

    The case $t_Q = n$ is trivial: as the height of $C$ is $n$, the upper bound of $l_Q$ under any replicated data placement function is $n$, so $t_Q$ cannot be violated.

    Finally, we consider the case $t_Q = n-1$. 
    If $r'$ changes the latency $l_Q$ compared to $r$, it must change the routing for causal access tree $C$.
    According to Def.~\ref{eqn:constrained}, this can only happen if a replica of an object in $C$ is placed together with its predecessor in a root-to-leaf path of $C$.
    As mentioned in the previous case, the upper bound of $l_Q$ is $n$.
    Modifying the routing means at least one object can be accessed at the same server as its predecessor.
    The upper bound on $l_Q$ becomes $n-1$, which is not larger than $t_Q$, a contradiction.
\end{proof}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/local_min_example.pdf}
    \vspace{-1\baselineskip}
    \caption{Example causal access trees. Co-optimized paths are highlighted in red. } 
    \label{fig:short_q_7}
    %\vspace{-1em}
\end{figure}


\begin{comment}
\spara{Making incremental updates robust}
To show how to enforce the robustness condition, we integrate it in the naive replication algorithm of Algorithm~\ref{algo:naive} and present the robust version in Algorithm~\ref{algo:cascading_proof}. 

\begin{algorithm}[t]
\input{algorithms/naive-robust.tex}
\end{algorithm}

We traverse each pair of vertices $v_i, v_{i+1}$ from root to leaf of $p$ and consume the latency budget if needed. 
In addition, at each step from $v_i$ to $v_{i+1}$, we record the \emph{index} of the first vertex of the current $i$-hop subpath.
Like in the previous algorithm, when the budget is depleted, we replicate the remaining vertices in $p$ to the last server $d(v_{p_i})$ the query accesses. 
Additionally, to ensure that robustness holds for the current $i$-hop subpath, we replicate each vertex $v_j$ in the $i$-hop subpath to all the master server of its preceding vertices in the subpath. 
No additional replicas are required to make robustness hold for the subsequent $j$-hop subpaths with $j>i$.
\end{comment}

==> sections/causal_access_tree.tex <==
%\section{Causal access hypergraph and the tradeoffs of replication design choices}
%In this section, we propose a data structure named \emph{causal access hypergraph} to model the data access dependencies of a query, and the tradeoffs of replication choices. 

%\subsection{Modeling Data Dependencies with Causal Access Hypergraph}
%To capture the data access dependencies of a query for making replication decisions, we transform the causal access graph of a query into a \emph{causal access hypergraph} $H$. 
%\begin{definition}[Causal Access Hypergraph]
%Consider a database consisting of a set of records $V$ and a query $q$. 
%The causal access hyerpgraph $H_q = (X, E)$ of $q$ consists of a set of hypernodes $X$ and edges $E$. 
%Each hypernode $x_{id, sid} \in X$ contains a subset of records ${v_1, v_2, ..., v_n} \in V$ such that the master copies of $v \in x$ are located at the same server $s_{sid}$, each $v \in V$ has te same set of causal relationships with other nodes in $x$, and each $v$ is required by the query.
%Each directed edge $e \in E$ is an ordered pair $E(x_1, x_2)$ of two hypernodes $x_1$ and $x_2$, which indicates the causal access sequence $x_1 \rightarrow x_2$. 
%\end{definition}

%\begin{algorithm}
%\centering
%\caption{Causal access hypergraph generation algorithm}\label{algo:transform_to_hypergraph}
%\begin{flushleft}
%\hspace*{\algorithmicindent} \textbf{Input: } Causal access graph $G=(V,E)$, data partitioning scheme $P : v \longrightarrow \{ s_1, s_2, ..., s_i \}$\\
%\hspace*{\algorithmicindent} \textbf{Output: } Causal access hypergraph $H=(X,E)$
%\end{flushleft}
%\begin{algorithmic}[1]
%\State $H \gets \{\}$
%\For{$v \in G.V$}
%  \State $x_{id,v.sid} \gets v$
%  \State $H.X \gets H.X \cup x_{id,v.sid}$
%\EndFor
%\State $H.E \gets G.E$
%\For{$E(x_{i,m}, x_{j,n}) \in H.E$}
%  \If{$m == n$}
%    \If{$x_{i,m}$ has a children $x_{l,o}$ where $m \neq o$}
%      \State $x_{k,m} \gets x_{i,m}$
%      \For {$x \in x_{i,m}.childern \setminus x_{j,n})$}
%        \State $H.E \gets H.E \cup E(x_{k,m}, x)$
%      \EndFor
%      \State $H.X \gets H.X \cup x_{k,m}$
%    \EndIf
%    \State $x_{i,m}.V \gets x_{i,m}.V \cup x_{j,n}.V$
%    \For {$x \in x_{j,n}.childern$}
%      \State $H.E \gets H.E \cup E(x_{i,m}, x)$
%    \EndFor
%    \State $H.X \gets H.X \setminus x_{j,n}$
%    \State $H.E \gets H.E \setminus E(x_{i,m}, x_{j,n})$
%  \EndIf
%\EndFor
%\Return $H$
%\end{algorithmic}
%\end{algorithm}

  
%We present the algorithm for transforming a causal access graph into a causal access hypergraph in Algorithm \ref{algo:transform_to_hypergraph}. 
%The intuition of the algorithm is as follows. 
%We merge two hypernode $x_1$ and $x_2$ into one if there exists a causal access relationship between $x_1$ and $x_2$, and they can be processed at the same server (i.e., $x_1.sid == x_2.sid$). 
%We duplicate the $x_1$ if there exists a childern $x_n$ of $x_1$ where $x_1.sid != x_2.sid$ to seperate the causal access relationship between $x_2$ and $x_n$.

%Algorithm \ref{algo:transform_to_hypergraph} first transform each vertex in the causal access graph $G$ into a hypernode with corresponding server id and add them to the causal access hypergraph $H$, and copy each edge in $G$ to $H$ (Line 1 - Line 5).  
%Then, for causal access relationship $E(x_{i,m},x_{j,n})$ that can be processed at the same server (Line 6 - Line 7), if $x_{i,m}$ has a remote child (Line 8), we create a duplication $x_{k,m}$ of $x_{i,m}$. (Line 9 - 11).
%We then add the duplication to the set of hypernodes in $H$ (Line 12). 
%After that, we merge $x_{j,n}$ into $x_{i,m}$ (Line 13 - Line 15). 
%Finally, we remove the childern node $x_{j,n}$ from the hypergraph (Line 16 - Line 17). 


%\begin{figure}[t!]
%  \centerline{\includegraphics[width=0.4\textwidth]{figures/causal_access_hypergraph.pdf}}
%  \caption{Causal access hypergraph of the running query example. }
%  \label{fig:causal_access_hypergraph}
%\end{figure}

%Figure \ref{fig:causal_access_hypergraph} shows the causal access hypergraph representation of the example query in Figure \ref{fig:causal_access_graph}. 
%The query starts at $Person_1$, which is located at $s_1$. 
%After processing $Person_1$, as the query will process $Person_3$ locally and process $Person_2$ remotely. 
%Therefore, we create two hypernodes $x_{1,1}$ and $x_{5,1}$ to seperate the two causal access relationships. 
%We group $Person_1$ and $Person_3$ into $x_{5,1}$ as they are both processed at $s_1$ and share the same set of causal relationship. 
%Similarly, we create two hypernodes $x_{2,2}$ and $x_{3,2}$ for $Person_2$ as the subsequent processing after $Person_2$ involves both local processing and remote processing. 
%The above causal access relationship between $Person_1$ and $Person_2$ are represented as two directed edges $E(x_{1,1}, x_{2,2})$ and $E(x_{1,1}, x_{3,2})$. 
%We then continue to construct the causal access hypergraph until all the data accesses of the query are captured. 

%Note that a hypernode is the unit of replication, as it is neceesary to totally remove the required data access at one server to save one inter-server hop.
%For example, consider $x_{2,2} \in H$. 
%If we only replicate $Person_2$ to the server of its parent hypernode $x_{1,1}$, although $Person_1$ and $Person_2$ can be retrieved at $s_1$, the query still needs to hop from $s_1$ to $s_2$ to retrieve $Message_4$. 
%When represented as a causal access hypergraph, the latency of a query equals to the length of the critical path in $H$. 


%\subsection{Replication Problem Definition}
%\nn{We assume that each of the query types can be modeled as a sequence of data accesses. }
%With the causal access hypergraph, we formally define our replication problem as follow. 
%\begin{definition}[Problem definition.]
%Given a dataset $D$, an initial data placement scheme $P$ which maps $d \in D$ to a set of servers $S$, a set of user-defined $n$-hop query types $Q_t$, and a hop budget $k$, 
%our goal is to come up with a replication scheme $R$ which maps $d \in D$ to a set of servers $S$, 
%such that the length of the critical path in the causal access hypergraph $H$ of each possible query instancea $q \in Q_t$ is $\leq k$, 
%the overall replication cost is minimized, 
%and the maximum memory utilization of all servers is minimized. 
%\end{definition}



%\subsection{Replication Design Choices}
%Given a causal access hypergraph that violates the $k$-hop guarantee, one straightforward solution is to enumerate all the possible replication schemes (i.e., consider replicating vertices in each hypernode to another server) and pick the one with the minimum cost. 
%For example, suppose we want to provide a 1-hop guarantee for the query example. 
%As the critical path $x_{1,1} \rightarrow x_{3,2} \rightarrow x_{4,1}$ has length equals to 2, we need to replicate vertices to eliminate one inter-server hop. 
%We may replicate all vertices $v \in x_{1,1}$ to its child server $s_2$, replicate all vertices $v \in x_{3,2}$ to its parent server $s_1$, replicate all vertices $v \in x_{4,1}$ to its parent server $s_2$, and so on.
%Replications can be divided into two types- \emph{downward replication} where replication is from parent node to its child server, and \emph{upward replication} where replication is from child node to its parent server. 
%Here, we discuss the tradeoffs of these two types of replication decisions. 



%\emph{Downward replication. } 
%Downward replication represents replication schemes that replicate a vertices in a parent hypernode to the server of its child hypernode. 
%In the running example, replicating all $v \in x_{1,1}$ to the server $s_2$ of its child hypernode $x_{3,2}$ is considered as a downward replication (red arrow in Figure \ref{fig:upward_downward_replication}). 
%Specifically, the replica of $Person_1$ will be created and stored at $s_2$.  
%Here, when we execute the example query, there are two possible locations to route the query to. 
%In particular, $s_1$ contains the master copy of $Person_1$, whereas $s_2$ contains the replica of $Person_1$. 
%However, only routing the query to $s_2$ will satisfy the \emph{k}-hop guarantee as $Person_1$ and $Person_2$ can be found on $s_2$, then the query will be routed to $s_1$ to retrieve $Message_5$. 
%On the other hand, if the query is routed to $s_1$, the query will not follow the previously optimized routing path, and needs to hop from $s_1 \rightarrow s_2 \rightarrow s_1$. 
%This implies that an additional routing table is needed to memorize the downward replication optimized route. 
%We need to maintain one entry per replica in the additional routing table to ensure the query will follow the desired path to satisfy the \emph{k}-hop guarantee. 
%In practice, the size of such routing table could exceed the capacity of the memory as the number of replicas needed to provide a \emph{k}-hop guarantee could be large depending on the set of user-defined query types. 
%In this case, we may need to fetch the neceesary routing information from disk, which will significantly increase the latency of the query. 
%Techinques such as query containment checking could reduce the size of the additoinal routing table. 
%However, it needs to be performed on query execution time and lower the performance of the query, which violates our assumption that the query types are latency critical. 

%\emph{Upward replication. }
%Upward replication represents replication schemes that replicate a vertices in a child hypernode to the server of its parent hypernode. 
%An upward replication example is shown in Figure \ref{fig:upward_downward_replication} (blue arrow). 
%In this replication scheme, we replicate $Person_2$ to the server of its parent hypernode $s_1$. 
%It presents an opportunity for us to couple the upward replication with a simple routing logic to replace the additional routing table.
%Specifically, for each next hop vertex $v_{next}$, the query executor first check whether $v_{next}$ exists in the local database. 
%If yes, the query will process $v_{next}$ locally, and continue until the next hop vertex does not exist in the local database.
%If not, the query executor routes the query to the server that contains the master copy of $v_{next}$. 
%Take the upward replication example in Figure \ref{fig:upward_downward_replication} as an example. 
%The query executor will first route the query to $s_1$ as it contains the master copy of the starting vertex $Person_1$. 
%After processing $Person_1$, the query executor will check whether the next hop vertex $Person_2$ exist locally. 
%Since the upward replication scheme created a replica in $s_1$, the query executor will continue to process $Person_2$ locally. 
%It will then check whether $Message_5$ exist locally. 
%Since it does not, the query executor will route the sub-query $Person \rightarrow Message$ with starting vertex $Person_2$ to the server $s_1$ which contains the master copy of the next hop vertex $Message_5$. 
%Finally, the query executor retrieves $Message_5$ at $s_1$, and return all results to the user. 
%By coupling the upward replication with the proposed query routing logic, the query does not need a routing table to memorize the routing decision to satisfy the \emph{k}-hop guarantee. 
%Therefore, our algorithm only considers upward replications to avoid burden of an additional routing table. 




%\subsection{"Follow your parent" constraint}
%Another constraint that we need to enforce is the "follow your parent constraint" \nn{need a better name}, which only allows hypernodes to be replicated to its closest non-replicated parent hypernode. 
%Suppose the user require $k = 1$.
%One can replicate $v_3 to v_5$ to $S_2$ to reduce one inter-server communication cost, and replicate $v_2$ to $S_1$ to reduce another communication cost. 
%However, although both replication can reduce one communication cost individually, the depth of the tree after implementing the whole replication plan is still two. 
%The reason is that after processing $v_1$, the server will continue to process the replica of $v_2$ locally. 
%Since $v_2$ is already processed at $S_1$, the query will not be routed to $S_2$ and the replicas $v_3$ to $v_5$ we created will not be useful. 
%Therefore, to make use of all the replicas, our algorithm only allows hypernodes to be replicated to its closest non-replicated parent hypernode, such that all replicas can be found at the non-replicated parent hypernode. 



%\subsection{Size of the query execution graph}
%To provide a $k$-layer guarantee, the intuitive way is to materialize the query execution graph (i.e., all possible query paths), analysis the data dependencies between data accesses, and generate a replication scheme with the global minimal cost \nn{or is it NP-hard?} such that all possible queries are within $k$. 
%However, the size of the query execution graph can be larger than the dataset itself. 
%Consider an extreme case where a dataset consists of $M$ people, and each person knows all other people.
%We can model the dataset as a data graph $G_M$, where each person is modeled as a vertex, and there exists an edge between two vertex $v_i$ and $v_j$ if person $i$ and person $j$ know each other. 
%Since each person knows all other person, $G_M$ is an $M$-clique. 
%Suppose the query type $Q_t$ is to find the $n^{th}$ hop friend given a starting person (i.e., $n$-hop query). 
%The number of possible query paths of $Q_t$ equals to the number of possible paths with length $n$ in $G_M$, which equals to $\prod\limits_{i=0}^{n-1} (|M| - i) = O(|M|^n)$. 
%As the size of the query execution graph grows exponentially with $n$, and $n$ is user-provided, the size of the query execution graph are unbounded. 
%To overcome this, our algorithm checks each possible paths individually to avoid materializing the query execution graph. 

==> sections/problem_definition-old.tex <==
\section{Problem Definition}
\label{sec:system-model}

\subsection{Modeling Multi-Hop Workloads}
In this subsection, we model both the dataset and the queries to model a multi-hop query workload.

\spara{Dataset}
We model a dataset $D$ as a set of abstract \emph{objects}.
This paper focuses on graph databases, and we primarily consider a vertex and its adjacency list as an object.
However, the model is generic and can be applied to other types of databases.

\spara{Queries}
Queries are modeled in terms of their data accesses and the causal dependencies of accesses.
Executing a query involves accessing multiple objects in the dataset.
If the access to an object $v$ \emph{causally precedes} the access to another object $u$ \emph{in the same query}, we say that $v$ happens before $u$, or $hb(v,u)$. 
Consider the example graph query of Figure~\ref{fig:multihop_example}.
Suppose the query starts by accessing a vertex $v$ associated with a person, called the root.
Only after accessing the adjacency list of $v$ can the query access the vertices $u_i$ associated to the people that $v$ knows. 
In this case, $hb(v,u_i)$.
The happen before property is transitive, that is, $hb(v,u)$ and $hb(u,z)$ implies $hb(v,z)$.

We model a sequence of causally-related data accesses as a \emph{causal access tree}, which we define as follows:
\begin{definition}[Causal access tree]
    A causal access tree $C$ over a dataset $D$ is a tree where each node is mapped to an object in $D$.
    A node $v_p$ is the parent of another node $v_c$ if and only if $hb(v_p,v_c)$ and there is no object $u \in D$ such that $hb(v_p,u)$ and $hb(u,v_c)$.
\end{definition}
%Note that the same object may appear multiple times in a causal access tree.

We model a \emph{query} $Q$ as a set of causal access trees and a \emph{workload} $W$ as a set of queries.
Each query in the workload can be modeled as one or more causal access trees.
%There are different possible ways to obtain causal access trees from an actual query workload, \red{as we will discuss later in the paper}.
This workload model is not specific to a query language or data representation.
It is a logical model that does not consider how data is physically stored in the cluster.
We now discuss how to model physical data placement.

\spara{Data placement}
The workload is executed by a system consisting of a set of servers $S$, each storing a partition of the dataset $D$.
Any distributed system must keep a \emph{data partitioning function} $d$, which maps each object of $D$ to one server.
Formally, given a dataset $D$ and a set of servers $S$, a data placement function is a function $d: D \rightarrow S$. 
This function is provided as an input to the problem.

\spara{Query execution and distributed traversals}
The system processes queries from clients.
A client sends a query to the coordinator server $d(v)$, where $v$ is the root of the causal access tree of the query.
If a query consists of multiple causal access trees, the client sends multiple subqueries to multiple coordinators.

The coordinator accesses objects in the order defined by the causal access tree $C$, starting from the root.
A distributed traversal is necessary whenever a server $s$ needs to access a remote object $u$, i.e., such that $d(u) = s' \neq s$.
In this case, $s$ sends a subquery to server $s'$ using a Remote Procedure Call (RPC). 
Server $s'$ continues accessing objects according to $C$ starting from the object $u$ on and responds to the RPC with the data subgraphs matching the subquery.
This process can be recursive, generating multiple nested RPC calls.
At the end of the query execution, the coordinator gathers all the accessed data, computes aggregations if required, and returns the result to the client.
The subquery shipping approach avoids repeatedly fetching data from remote servers and maximizes data access locality at the remote server whenever possible.
RPCs are also used in RDMA-enabled graph databases because of their better data locality compared to repeated RDMA fetches ~\cite{A1}.
%For example, work on the Pragh ~\cite{Pragh} system, which is RDMA-enabled, conducted a performance comparison between local 2-hop query processing and distributed 2-hop query processing with RDMA. 
%The results show that running 2-hop queries in an 8-node RDMA-capable cluster can only achieve less than 4\% throughout local query execution. 

The latency of a distributed traversal is expressed by a \emph{latency function} $l$.
We consider a homogeneous cluster, where $l(s_1, s_2)$ is equal to $1$ if $s_1 \neq s_2$, or $0$ otherwise. 
We measure latency in terms of the number of nested RPCs required to return the result. 



\spara{Query latency}
The causal dependency information captured by the causal access tree is important to understanding the latency cost of a query.
Causally-dependent accesses must be executed sequentially, whereas non-causally-dependent ones can be executed in parallel.
In Figure~\ref{fig:example_query}, accessing a user happens before accessing the friends of that user, and accessing the friends happens before accessing their messages.
It is possible to access multiple friends of a user in parallel, but we must first access the user to know which set of friends should the query access.
Therefore, the latency cost of the query is equal to the maximum cost of matching any root-to-leaf path in its causal access trees.
    

\begin{definition}[Latency cost of a path]
    Let $D$ be a dataset, $C$ a causal access tree over objects in $D$, $p = \langle v_{p_1}, \ldots,  v_{p_n}\rangle$ a path between two nodes in $C$, $d$ a data placement function from $D$ to a set of servers $S$, and $l$ a latency function over $S$.
    The latency cost $h(p)$ of $p$ is defined as:
    \begin{equation}
        h(p) = \sum_{(v_{p_i},v_{p_{i+1}}) \in p} l(d(v_{p_i}),d(v_{p_{i+1}})) 
    \end{equation}
\end{definition}

\begin{definition}[Latency cost of a query]
    Let $Q = \{C_1,\ldots,C_m\}$ be a query over a dataset $D$, $P_i$ the set of all root-to-leaf paths in the causal access tree $C_i \in Q$.
    The latency cost $l_Q$ of $Q$ is defined as:
    \begin{equation}
        l_Q = \max_{C_i\in Q} \Big(\max_{p \in P_i} h(p) \Big) \label{eqn:cost}
    \end{equation}
\end{definition}

\subsection{The Latency-Bound Replication Problem}

We have modeled the latency of distributed multi-hop queries in a system without replicas.
This paper addresses the problem of reducing latency by replicating data.
We describe how the latency cost of a query changes in the presence of replicas in the following.

\spara{Data replication and query routing}
Besides the master copy of a vertex, we consider additional replicas.
We first define a \emph{replicated data placement function} $r$ that maps each vertex $v$ to a set of servers, one of which is the location of its master copy $d(v)$.

\begin{definition}[Replicated data placement function]
    Given a dataset $D$, a set of servers $S$, and a data placement function $d$, a replicated data placement function $r$ extending $d$ is a function $r: D \rightarrow 2^S$ such that $\forall v \in D, d(v) \in r(v)$.
\end{definition}

A query that accesses a data vertex $v$ can now be \emph{routed}, through a distributed traversal, to any server having a copy of $v$.
We introduce a routing function to model these routing choices and associate each vertex in a causal access tree to a specific copy.

\begin{definition} [Routing function]
    Let $C$ be a causal access tree and $r$ a replicated data placement function.
    A routing function $a_r$ under $r$ associates each node $v$ in $C$ with a server $a_r(v) \in r(v)$.
\end{definition}

Routing a query to different servers with a copy of the required vertex may lead to different latency costs.
The latency cost of a query with replicas is defined similarly to Eqn.~\ref{eqn:cost}.
However, for every causal access tree, we are now required to route the (sub)query to the servers that leads to the overall minimum latency cost.

\begin{definition}[Latency cost of a path with replication]
    Let $D$ be a dataset, $C$ a causal access tree over objects in $D$, $p = \langle v_{p_1}, \ldots,  v_{p_n}\rangle$ a path between two nodes in $C$, $r$ a replicated data placement function over a set of servers $S$, $l$ a latency function over $S$, and $a_r$ a routing function under $r$.
    The latency cost $h(p, a_r)$ of $p$ under $a_r$ is defined as:
    \begin{equation}
        h(p, a_r) = \sum_{(v_{p_i},v_{p_{i+1}}) \in p} l(a_r(v_{p_i}),a_r(v_{p_{i+1}})) 
        \label{eqn:latency-subpath-repl}
    \end{equation}
\end{definition}

\begin{definition}[Optimal latency cost of a query with replication]
    Let $Q = \{C_1, \ldots, C_m \}$ be a query over a dataset $D$, $P_i$ the set of all root-to-leaf paths in the causal access tree $C_i \in Q$, $r$ a replicated data placement function, and $A_r$ the set of all possible routing functions under $r$.
    The optimal latency cost $l_Q$ of $Q$ under $r$ is defined as:

\begin{equation}
    l_Q = \max_{C_i\in Q} \Big(\max_{p \in P_i} \Big(  \min_{a_r \in A_r} h(p, a_r) \Big)\Big)
    \label{eqn:latency-cost-repl}
\end{equation} 
\end{definition}

Replication results in additional storage cost, which we aim to minimize. 
Also, we aim to balance the storage costs among servers.
Suppose the storage cost of a vertex $v$ and its adjacency list is $f(v)$.

\begin{definition}[Data storage cost]
    Let $D$ be a dataset, $S$ a set of servers, $f$ a storage cost function, and $r$ a replicated data placement function. The data storage cost $f_r (s)$ of $r$ for a server $s \in S$ is defined as:
    $$
        f_r(s) = \sum_{v \in D:\: s \in r(v)} f(v)
    $$
\end{definition}

\spara{Problem definition}
We formally define the problem addressed in this paper.
The problem is to find a replicated data placement function $r$ that guarantees all queries complete within their latency constraints (first constraint) and the storage costs among all servers are balanced (second constraint) while the total replication cost is minimized (minimization problem).
Implicit in the problem definition is to find a routing function $a_r$ for each causal access tree $C$ of a query $Q$ that minimizes the latency function $l_Q$, as defined in Eqn.~\ref{eqn:latency-cost-repl}.

\begin{definition}[Latency-bound replication problem]
    Let $D$ be a dataset, $W = \{Q_1, \ldots, Q_m\}$ a workload consisting of a set of queries, each associated with a latency constraint $t_{Q_i}$, $S$ a set of servers, $d$ a data placement function, $l$ a latency function, $f$ a storage cost function, $M_s$ the storage capacity of a server $s$, and $\epsilon$ a load imbalance constraint.
    The latency-bound replication problem is to find a replicated data placement function $r$ extending $d$ such that:
    \begin{equation}
        \begin{aligned}
            \min_r \quad & \sum_{s \in S} f_r(s) \\
            \textrm{s.t.} \quad & \forall Q_i \in W: \: l_{Q_i} \leq t_{Q_i} \quad \wedge\\
            & \forall s, s' \in S:\: |f_r(s) - f_r(s')| \leq \epsilon   \\
            & \forall s \in S, f_r(s) \leq M_s\\
        \end{aligned}
        \label{eqn:problem}
    \end{equation}
\end{definition}

\begin{theorem}
    The latency-bound replication problem is NP-hard.
\end{theorem}
\begin{proof}
    The proof is in two steps. 
    In the first step, we reduce the problem to a problem we call \emph{Min-bridge bisection problem}.
    In the second step, we reduce that problem to the min-bisection problem for 3-regular graphs, that has been proven to be NP-hard~\cite{bui1987graph}.

    \emph{Step 1.}
    The min-bridge-vertex bisection problem is defined as follows: given a graph $G = (V_G, E_G)$ with $2n$ vertices, partition its vertices into two sets of $n$ vertices each such as the number of ``bridge vertices'' is minimized, where a bridge vertex is a vertex in one partition having at least one neighbor in the other partition.

    We now build an instance of the latency-bound replication problem as follows.
    First, we build a dataset $D$ and a workload $W$.
    For each vertex $v \in V_G$, we add two objects to $D$: a \emph{regular} object $v_o$ and a \emph{marker} object $v_m$.
    We also add a query to $W$ with the following causal access tree: $v_m$ is the root and it is parent to $v_o$.
    In turn, $v_o$ is parent of the regular object $u_o$ for each vertex $u \in N(v)$.
    The storage cost function $f$ is such that $f(v_m) = 1$ for each marker object and $f(v_o) = \epsilon/n$ for each regular object, where $\epsilon < 1$ is the load balancing constraint of Eqn.~\ref{eqn:problem}.
    The maximum storage of servers are $M_{s_1} = M_{s_2} = n+\epsilon$ and $M_{s_3} = M_{s_4} = n+2\epsilon$.
    The data partitioning function $d$ is defined as follows.
    We have four servers.
    Servers $s_1$ and $s_2$ contain the marker objects for half of the vertices in $V_G$ each.
    Server $s_1$ also contains the regular objects for the vertices whose markers are in $s_2$ and vice versa.
    The latency bound for all queries is $0$.

    We now establish some properties about the solution of this instance of the latency-bound replication problem.
    The root of every causal access tree is a marker object. 
    Without replication, the marker of a vertex and its regular object are located on two different servers.
    Accessing a marker at server $s_1$ or $s_2$ will result in a subsequent distributed traversal to the regular object, which would violate the latency bound.
    Therefore, we need to add replicas to servers $s_3$ and $s_4$ since $s_1$ and $s_2$ have already reached their maximum storage capacity.
%    \ms{If we don't want to indicate an extra capacity per server, we can fill up $s_1$ and $s_2$ with ``null'' objects that are not accessed by any causal access tree. These vertices will not have to be replicated on  $s_3$ and $s_4$}
    The load balancing constraint and maximum storage constraints of Eqn.~\ref{eqn:problem} requires that $s_3$ and $s_4$ have replicas for no more than half of the marker objects each plus replicas of any number of regular objects.
    
    An optimal solution to the latency-bound replication will assign half of the markers to $s_3$ and $s_4$ each to minimize the replicas of the regular objects.
    The latency constraint requires that a marker of a vertex is co-located with the regular object of that vertex and the regular objects of all its neighbors.
    In this solution, the storage cost for $s_3$ and $s_4$ is in $[n+\epsilon, n+2\epsilon]$, which respects both the load balancing and storage capacity constraints.
    
    Consider now a bisection of the original graph $G$ where each vertex is assigned to partition $V_1$ (resp. $V_2$) based on whether its marker is stored on $s_3$ (resp. $s_4$) in the optimal solution of the latency-bound replication problem.
    We claim that this bisection is optimal for the min-bridge bisection problem.
    Without loss of generality, suppose that a vertex $v$ in $V_1$ has at least one neighbor $u$ in $V_2$.
    This means that the regular object of $u$, which is already stored at $s_4$, must be also replicated at $s_3$, incurring an additional storage cost that would not be necessary if both $v$ and $u$ were in the same partition.
    This cost must be paid only once for all neighbors of $u$ in $s_3$.
    Vertex $u$ is a bridge vertex and the extra storage cost to replicate it is paid only once for all its neighbors in the other partition.
    Whether this cost is paid depends on how the solution splits the marker vertices between $s_3$ and $s_4$, which also determines which vertices are bridges in the corresponding bisection $(V_1,V_2)$.
    An optimal solution to this instance of the latency-bound replication problem minimizes the replication cost and thus also minimizes the number of bridge vertices of the corresponding bisection $(V_1,V_2)$.
    
    \emph{Step 2.}  Given a 3-regular graph $G$ with $2n$ vertices, construct a graph $H$ by replacing each vertex $v$ by three copies $v_1,v_2,v_3$, each attached to one of the edges of $v$ and having edges to the other two copies. 
    The graph $H$ has $6n$ vertices and is also 3-regular.

	Now we claim that $G$ has a bisection of size $K$ if $H$ has a bridge bisection of size $K$.

	Suppose that $G$ has a bisection of size $K$, and the vertex partition of $G$ is $(V_1,V_2)$, each of $n$ vertices, then form the vertex partition $(U_1,U_2)$ of $H$ by the following: for each vertex $v$ in $V_1$, add all 3 copies to $U_1$. Clearly, since there are $K$ edges crossing $(V_1,V_2)$, there are $K$ bridge vertices in $(U_1,U_2)$, each correspond to a crossing edge of $(V_1,V_2)$.

	Suppose that $H$ has a bridge bisection $(U_1,U_2)$ of size $K$. 
	First, we claim that all copies of every vertex $v$ in $G$ must be in one side of $H$. 
	The idea for the proof is that, if copies of the same vertex in two sides, for example $v_1$, $v_2$ are in $U_1$ while $v_3$ in $U_2$, then there must be another vertex, say $w$, whose copies are in different sides of the partition (say $w_1$ in $U_1$ while $w_2$ and $w_3$ are in $U_2$). 
	We then swap $v_3$ to $U_1$ and $w_1$ to $U_2$. 
	The resulting partition remains balanced, and keep doing that until all copies of every vertex is in one side of $H$. 
	It’s not hard to see that the swapping operation does not increase the number of bridge vertices.

	Now, as all copies of every vertex is in one side of $(U_1,U_2)$, by simply replacing these copies with the original vertex, we obtain a bi-partition $(V_1,V_2)$ of $G$. 
	The number of crossing edges will be the number of bridge vertices because each bridge vertex is incident to exactly one edge crossing $(U_1,U_2)$. 
	Thus, $G$ has a bisection of size $K$.
\end{proof}

\section{Distributed query routing}
In this section, we argue that query routing with replicas may require additional routing tables that can be larger than the dataset.
Therefore, we consider a constrained version of our problem where the routing function is \emph{thrifty}, i.e., it does not use any extra routing information.
In this case, we show that any optimal replicated data placement function satisfies a property called \emph{upward replication}.
We can then restrict our search to solutions with that property.

\subsection{Thrifty Routing}
When a query needs to perform a distributed traversal, the server must route the subquery to a remote server storing the object that needs to be accessed next.
When there is only one copy of each object stored in the system, the data placement function $d$ indicates the server storing that copy.
However, with replicas, there may exist more than one candidate routing destination. 
The query executor must choose a server that respects the query's latency constraint as the routing destination. 
This may require additional routing information that is in proportion to the number of causal access trees in the workload, as we show with an example in Figure~\ref{fig:upward_downward_replication}.

% \subsection{Old Text}
% As the data is partitioned across servers, the required next-hop vertex of a query may not exist locally, and the query executor needs to route the subquery to a server containing the required data to continue the execution. 
% With replicas, this process may require additional routing information that is large in size. 
% First, the system needs to maintain an additional table at each server that stores the locations of replicas to know the set of candidate routing destinations. 
% The number of entries in the table is in proportion to the number of replicas in the system, which is potentially large in size. 
% Second, routing a query to different servers may lead to different latency costs. 
% Distributed query routing in a system without replicas is trivial since there only exists one candidate routing destination (i.e., the master copy).
% However, with replicas, there may exist more than one candidate routing destination. 
% The query executor must choose a server that respects the query's latency constraint as the routing destination. 
% This may require additional routing information that is in proportion to the number of matches of queries in the workload, as we show with an example in Figure~\ref{fig:upward_downward_replication}.

%In the existing work that introduces replicas such that queries can be processed at a single server, the system can simply memorize the optimized location to execute each query. 
%Such storage cost can be avoided by always routing the query to the master copy of its starting vertex and adding replicas on that server \cite{SPAR}. 

% Routing of queries becomes tricky, as routing it to different locations may lead to different latency costs for the same query.
% We illustrate the idea in Figure \ref{fig:upward_downward_replication}. 
Consider an example data graph $G$ in Figure \ref{fig:up_down_G}.
The color of a vertex denotes its type.
Suppose the system executes query $Q$ in Figure \ref{fig:multihop_example}.
%Assume that all pairs of servers has a latency cost of 1. 
%$Q$ starts from a green vertex, access its green vertex neighbors, and accesses its corresponding yellow vertex neighbors. 
There are two causal access trees of $Q$ in $G$, corresponding to the two green vertices $v_2, v_4$ matching the root vertex of $Q$. 
The system first sends $Q$ to server $s_1$ and $s_2$. 
The query executor at $s_1$ accesses $v_2$, then proceeds to access $v_2$'s outgoing green neighbor $v_4$. 
As vertex $v_4$ is not locally available at $s_1$, the query requires a distributed traversal to access it. 

Suppose $v_4$ is originally stored at $s_2$ and replicated at $s_3$ (see Figure~\ref{fig:downward_replication}).
Routing to either server can access $v_4$ but will lead to different query latency. 
If the distributed traversal is routed to $s_3$, the query executor at $s_3$ can access both $v_4$ and its yellow neighbor $v_6$ locally. 
However, if the distributed traversal is routed to $s_2$, another distributed traversal to $s_3$ is necessary to access the yellow vertex $v_6$, resulting in a higher latency cost. 
If the latency constraint allows only one distributed traversal, only routing to $s_3$ is admissible. 

In this example, server $s_1$ needs to store an additional routing table to memorize the above routing information for this causal access tree $C$.
The additional routing table may be large because it may need separate entries for each causal access tree.
Suppose that server $s_1$ executes another query with a causal access tree $v_3 \rightarrow v_4 \rightarrow v_5$.
Server $s_1$ accesses $v_3$, then needs to perform a distributed traversal to access $v_4$.
In this case, however, it is necessary to route the distributed traversal to $s_2$ instead of $s_3$ to ensure only one distributed traversal is required.
This example shows that the additional routing table at $s_1$ needs to have multiple entries for the remote vertex $v_4$, one for each causal access tree.
% In the running example, $s_1$ has to maintain an additional routing table with an entry for $M$ with the root vertex $v_2$, such that the subquery is routed to the server that leads to the lowest latency cost of $Q$. 
% Different matches may require separate entries even when they refer to the same query. 
% For example, suppose that $v_4$ has another yellow neighbor $v_9$ located at $s_2$.
% This would introduce another match for $Q$ consisting of the vertices $\langle v_2, v_4, v_9 \rangle$.
% To access this match, the quer
% The match $M'$ should be routed to $s_2$ to match $v_4$, unlike $M$ that is routed to $s_3$.
The size of the additional table grows in proportion to the number of causal access trees and may become larger than the dataset in the worst case.
%Furthermore, finding the optimal routing for each match may become a bottleneck as it requires examining each possible routing path.

%\ms{Maybe we could change the diagram to include $M'$.}
% If the size of the table exceeds the memory capacity, the query executor needs to fetch the necessary routing information from the disk, which significantly increases the latency of the query. 
% Techniques such as query containment checking \nn{cite} could reduce the size of the additional routing table. 
% Yet, the containment check needs to be performed at query execution time and lower the performance of the query, which violates our assumption that the query types are latency-critical. 

%Note that this problem does not arise in the special case when the latency budget of a query $Q$ is always equal zero, as assumed by some existing work \cite{MorphoSys,SPAR}.
%In this case, all vertices in a match of $Q$ must locate at the same server.
%No inter-server communication, and thus routing tables, are needed. 

\begin{figure}[t!]
    \centering
    % \hspace*{-3cm}
    % \begin{subfigure}[b]{0.20\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figures/upward_downward_Q.pdf}
         
    %     \caption{Query $Q$}
    %     \label{fig:up_down_Q}
    % \end{subfigure}
    % \newline
    % \hfill
    \begin{subfigure}[b]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/upward_downward_G.pdf}
        \caption{Dataset graph.}
        \label{fig:up_down_G}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.31\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/downward_replication.pdf}
        \caption{Routing with arbitrary replication.}
        \label{fig:downward_replication}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/upward_replication.pdf}
        \caption{Thrifty routing + upward replication.}
        \label{fig:upward_replication}
    \end{subfigure}
        \vspace{-0.5\baselineskip}
       \caption{Examples of possible routing paths under different replication decisions. Replicas are represented in solid colors. Routing paths are represented as dashed arrows. }
       \label{fig:upward_downward_replication}
       \vspace{-1em}
\end{figure}

\spara{Thrifty routing}
To avoid storing additional routing tables, we propose the following \emph{thrifty routing} logic: if a required object $v$ does not exist in the local storage of a server, the query executor at that server routes the distributed traversal to the master copy of $v$, which is $d(v)$.
Checking if a master or replica copy of $v$ is stored locally does not require any routing information, and any distributed storage system must already keep routing information to locate the master copy of every object.
Therefore, thrifty routing does not require any additional routing table. 

Formally, thrifty routing is equivalent to constraining the set of data copies that can be selected by the annotation function $a_r$.

\begin{definition}[Thrifty routing function]
    Let $C$ be a causal access tree, $p$ a root-to-leaf path in $C$, and $r$ a replicated data placement function. A thrifty routing function $a_r$ of $C$ under $r$ is defined for a node $v\in C$ as:
    \begin{equation*}
    a_r(v) = \left\{
    \begin{array}{rl}
      a_r(u) & \text{if } \exists u \text{ parent of } v \text{ in } p \wedge a_r(u) \in r(v),\\
      d(v) & \text{otherwise}.
    \end{array} \right.       
    \end{equation*}
    \label{eqn:constrained}
    \vspace{-1em}
\end{definition}
Beyond eliminating the need for additional routing tables, the thrifty routing function obviates the need for finding the routing function with the minimal latency cost in Eqn.~\ref{eqn:latency-cost-repl}, as we show next. \ms{Route to a server in $r(v)$ initially. This would make the NP-hardness proof still valid.}

\begin{lemma}\label{lemma:2_17}
    Given a replicated data placement function $r$ and a causal access tree $C$, there exists only one thrifty routing function. 
\end{lemma}

\begin{proof}
    We prove that $a_r(v)$ can only have one possible value for each node $v$ in $C$.
    The proof is by induction on the depth of a node $v$ in $C$.
    If $v$ is the root of $C$, then $a_r(v) = d(v)$ according to Def.~\ref{eqn:constrained}.
    In the inductive case, $v$ is the child of a node $u$.
    By induction, $a_r(u)$ has only one possible value, so also $a_r(v)$ has only one possible value according to Def.~\ref{eqn:constrained} based on whether $a_r(u) \in r(v)$.
\end{proof}

This Lemma leads to the following Corollary:

\begin{corollary}
    With thrifty routing functions, it holds that $A_r$ contains only one function $a_r$ and Eqn~\ref{eqn:latency-cost-repl} becomes:
    \begin{equation}
        l_Q = \max_{C_i\in Q} \Big(\max_{p \in P_i}\, h(p, a_r) \Big)
        \label{eqn:latency-space-optimal}
    \end{equation}
\end{corollary}

% \begin{proof}
%     We proof Lemma \ref{lemma:2_17} by induction.
%     Consider any root-to-leaf path $p$ of $M$ of length $k$. 
%     For the base case $k = 1$, $p$ only contains a root vertex $v_r$. 
%     By Eqn.~\ref{eqn:constrained}, there only exists one $a_M$ of $v_r$ and $a_M(v_r) = d(v_r)$ as there does not exist a parent vertex $u$ of the root vertex $v_r$ in $p$.
%     For the induction step, suppose $p$ of length $k$ only has one annotation function.
%     We extend $k$ to $k+1$ by adding one child vertex $v_i$ to the leaf vertex $v_l$ of $p$. 
%     As there must exist a parent vertex $v_l$ for $v_i$, $a_M(v_i)$ is determined by whether $a_M(v_l) \in r(v_i)$ as defined in Eqn.~\ref{eqn:constrained}. 
%     Therefore, by mathematical induction, there exists only one annotation function for any root-to-leaf path of $M$, and thus there exists only one annotation function for $M$.  
% \end{proof}

\spara{Upward replication function}
We describe a class of functions, namely \emph{upward replication functions}, that includes all optimal solutions to the latency-bound replication problem when using thrifty routing.
This restricts the space for solutions to the problem.

\begin{definition}[Upward replication function]
    Let $D$ be a dataset and $W = \{ Q_1, \ldots, Q_m\}$ be a workload consisting of a set of queries.
    A replicated data placement function $r$ is an upward replication function if the following holds: $a_r(v) \neq d(v)$ for some causal access tree $C$ of a query $Q_i\in W$ in $G$ implies $a_r(u) = a_r(v)$ for the parent $u$ of $v$ in $C$.
    \label{def:upward_replication}
\end{definition}

\begin{comment}
We define upward replication functions by construction: we start from an initial configuration where there is no replication, so $r=d$, and incrementally add one replica of a server at a time.
Formally, we call the step of adding one replica a \emph{replication update} and define it as follows:

\begin{definition}[Replicated data placement function update]
    Given a replicated data placement function $r$ on a set of server $S$ and a data graph $G = (V,E)$,
    a replicated data placement function $r_{v'}$ is an update of $r$ for some vertex $v' \in V$ if and only if it holds that: 
    $r_{v'}(v') = r(v') \cup \{s\}$ for some $s \in S \setminus r(v')$ and $\forall v \in V, v \neq v': r(v) = r_{v'}(v)$. 
\end{definition}

An \emph{upward replication update} is a special class of replication update that only add a replica of a vertex $v'$ to a server $s$ only if, for some match $M$, $v'$ is the descendant of $v$ in the causal access tree $C_M$ and server $s$ has a local copy of a vertex $v$.

\begin{definition}[Upward replication update]
    Let $Q$ be a query, $G$ a data graph, $r$ a replicated data function, and $r'$ and an updated replication function $r_{v'}$ of $r$ for $v'$.
    We say that $r_{v'}$ is an upward replication update if and only if there exists some match $M$ with causal access tree $C_M$ such that for some ancestor \ms{or parent?} vertex $v$ of $v'$ in some path $p$ of $C_M$ it holds $|r_{v'}(v') \setminus r(v')| = a_M(v)$. 
    \label{def:upward_replication}
\end{definition}

An \emph{upward replicated data placement function} is defined by construction as follows.

\begin{definition}[Upward replicated data placement function]
    A replicated data placement function $r$ is an upward replicated data placement function given an initial data placement $d$ if and only if it can be obtained by applying a sequence of upward replication updates on $d$.   
\end{definition}
\end{comment}

An example of an upward replication function is shown in Figure~\ref{fig:upward_replication}.
%Given a root-to-leaf path $p$ of a causal access tree, Upward replication updates only replicate child vertices to the server of their parent vertex in $p$. 
Replicating $v_6$ onto $s_2$ satisfy the definition because when matching $\langle v_2, v_4, v_6\rangle$, the query executor accesses $v_4$ at $s_2$ before $v_6$.
 %replicating $v_6$ to the server of its parent node $v_4$'s server $s_2$, and replicating $v_4$ to its parent server $s_1$ are considered as upward replication updates. 

We prove that any optimal solution to the latency-bound replication problem must be an upward replication function. 

\begin{theorem}
    In a system using thrifty routing, any optimal replicated data placement function solving the latency-bound replication problem is an upward replication function. 
\end{theorem}
\begin{proof}
    If an optimal replicated data placement function $r$ contains no additional object replicas compared to $d$, the proof follows directly from Def.~\ref{def:upward_replication}.
    If not, a replicated data placement function $r$ is optimal according to  Eqn.~\ref{eqn:problem} if and only if removing any object replica increases the latency of some query.
    This implies that each object replica must be accessed in some causal access tree.
    Formally, for each replicated object $v \in D$ and for each location of the replica $s \in r(v) \setminus \{d(v)\} $, 
    there must exist some causal access tree $C'$ of a query $Q\in W$ such that $a_r(u) = s$ for the parent $u$ of $v$ in $C'$.
    %there must be a parent $u$ of $v$ in some causal access tree $C'$ of a query $Q\in W$ such that $a_r(u) = s$ .
    
    Let $v$ be a replicated object in $D$ and $s$ be one of the servers where it is replicated.
    Assume that the system uses a thrifty routing function.
    We now show that any optimal replicated data placement function $r$ is an upward replication function, which according to Def.~\ref{def:upward_replication} implies that there exists some causal access tree $C$ such that $a_r(u) = a_r(v) = s$ for the parent $u$ of $v$ in $C$.
    
    Assume by contradiction that there exists no such $u$ for some replicated object $v \in D$.
    This means that for all causal access tree $C$ that accesses the replicated object $v$, if $a_r(v) = s$, $a_r(u) \neq a_r(v)$ for the parent $u$ of $v$ in $C$.
    By hypothesis, $a_r$ is a thrifty routing function.
    According to Def.~\ref{eqn:constrained}, if $a_r(u) \neq a_r(v)$, then $a_r(v) = d(v)$, and this holds for all causal access trees $C$ that includes $v$.
    However, this contradicts our previous finding that $a_r(v) = s \neq d(v)$ for some causal access tree $C'$.
\end{proof}

%\spara{Types of data replication}
%To discuss how data replication impacts query routing we use an example.
%\ms{should use $\hat{l}$ instead of $l$. Maybe we can change the notation to avoid using the hat all the time.}
%Consider the example data graph $G$ and query $Q$ in Figure \ref{fig:upward_downward_replication}. 
%The color of the vertex represents the type of the vertex. 
%Specifically, $Q$ starts from a green vertex, access its green vertex neighbors, and access its corresponding yellow vertex neighbors. 
%In this example, $Q$ has one causal access tree $v_2 \rightarrow v_4 \rightarrow v_6$ in $G$. 
%Suppose $l(s_1,s_2) = l(s_2,s_3) = 1$, $l_Q = l(d(v_2), d(v_4)) + l(d(v_4), d(v_6)) = 2$. 
%We further suppose the latency budget $t$ for $Q$ is 1, which means $Q$ violates the latency budget and requires replication to reduce its latency cost.  
%As the query always starts with the master copy of the vertex, %we can only replicate $v_4$ or $v_6$ to reduce the number of server hops of $Q$. 
%In particular, there are three feasible replication choices: replicating $v_4$ to $s_1$, replicating $v_4$ to $s_3$, or replicating $v_6$ to $s_2$. 

%In the following, we define two classes of data replication- namely \emph{downward replication update} and \emph{upward replication update}, and discuss the tradeoffs of adopting these two types of replications in practice. 
%Before that, we formalize how replication functions are incrementally updated by replicating a vertex $v'$ into a server.

%\begin{definition}[Replicated data placement function update]
%    Given a replicated data placement function $r$ and 
%    a data graph $G = (V,E)$,
%    a replicated data placement function $r_{v'}$ is an update of $r$ for some vertex $v' \in V$ if and only if it holds that: 
%    $r_{v'}(v') = r(v') \cup \{s\}$ for some $s \not\in r(v')$ and $\forall v \in V, v \neq v': r(v) = r_{v'}(v)$. 
%\end{definition}

%We can now formalize the two classes of data replication.

%\begin{definition}[Downward  replication update]
%Given a query $Q$, a data graph $G$, a root-to-leaf path $p$ in the causal access tree of $Q$ in $G$, a replicated data function $r$, a replication decision is classified as downward replication if it adds a replica $v_i$ at the server $d(v_j)$ to $r$, where $v_i, v_j \in p$ and $i < j$. 

%Given a query $Q$, a data graph $G$, a root-to-leaf path $p$ in a causal access tree of $Q$ in $G$, a replicated data function $r$, and an updated replication function $r_{v'}$ of $r$ for $v'$, $r_{v'}$ is a downward replication update if and only if for some vertex $v$ following $v'$ in $p$ it holds $|r_{v'}(v') \setminus r(v')| = d(v)$. 

%\end{definition}

%Downward replication updates replicate a parent vertex to the server of its child vertex. 
%In this example, replicating $v_4$ to $s_3$ is considered as a downward replication update, as shown in Figure \ref{fig:downward_replication}.  
%After the downward replication update, when the system receives the query $Q$ from a client library, the query executor at $s_1$ first processes the root vertex $v_2$. 
%Then, the query executor continues to process $v_4$, but the local storage at $s_1$ does not contain the target vertex. 
%The query executor has two possible destinations to route the subquery, as $s_2$ and $s_3$ both contains $v_4$. 
%However, only routing the query to the optimized path $s_3$ can reduce the latency cost since $v_4$ and $v_6$ can both be found on $s_3$ and does not require future server hops. 
%On the other hand, if the query is routed to $s_2$, the query needs to hop from $s_1 \rightarrow s_2 \rightarrow s_3$ to retrieves all vertices, which leads to $l_Q = 2$.
%This example shows that to make the correct routing decision after replication, the query executor needs to maintain an additional routing table to store the metadata and memorize the optimized route. 
%However, the size of such a routing table may exceed the memory capacity as the number of replicas created may be significant, depending on the set of user-defined queries and the latency budgets. 
%The query executor may need to fetch the necessary routing information from the disk, which significantly increases the latency of the query. 
%Techniques such as query containment checking \nn{cite} could reduce the size of the additional routing table. 
%Yet, it needs to be performed on query execution time and lower the performance of the query, which violates our assumption that the query types are latency-critical. 

%\begin{definition}[Upward replication update]
%    Given a query $Q$, a data graph $G$, a root-to-leaf path $p$ in a causal access tree of $Q$ in $G$, a replicated data function $r$, and an updated replication function $r_{v'}$ of $r$ for $v'$, $r_{v'}$ is an upward replication update if and only if for some vertex $v$ preceding $v'$ in $p$ it holds $|r_{v'}(v') \setminus r(v')| = d(v)$. 
%\end{definition}

%\begin{definition}[Upward replicated data placement function]
%    An upward replicated data placement function $r$ is a replicated data placement function that can be obtained as the result of applying a sequence of upward replication updates on the initial data placement function $d$.    
%\end{definition}

%Upward replication only replicates child vertices to the server of their parent vertex. 
%In this example, replicating $v_6$ to the server of its parent node $v_4$'s server $s_2$, and replicating $v_4$ to its parent server $s_1$ are considered as upward replication decisions. 

%\spara{Query routing}
%In this work, we combine upward replication updates with a constrained definition of the routing logic in the query executor to avoid the need of an additional routing table to follow the optimized paths.
%Specifically, we constrain $r$ to only allow upward replications for any root-to-leaf path. 
%At query execution time, if after matching a vertex $v$ at a server $s$ the next hop vertex $u$ does not exist in the local storage of $s$, the query executor routes the subquery to the master copy of the next hop $u$.
%This is equivalent to constraining the set of replicas that can be selected for a vertex by the annotation function $a_M$.

%\begin{definition}[Constrained annotation function]
%    Given a query $Q$, a data graph $G$, a root-to-leaf path $p$ in a causal access tree of $Q$ in $G$ with annotation function $a_M$, and an upward replicated data placement function $r$, $a_M$ is constrained if and only if for it holds that:
%    \begin{equation}
%    a_M(v) = \left\{
%    \begin{array}{rl}
%      a_M(u) & \text{if } \exists u \text{ parent of } v \text{ in } p \wedge a_M(u) \in r(v),\\
%      d(v) & \text{otherwise}.
%    \end{array} \right.       
%    \label{eqn:constrained}
%    \end{equation}
%\end{definition}

%\begin{lemma}\label{lemma:2_17}
%    Given a replicated data placement function $r$ and $M$ a partial or full match of $Q$ in $G$, there exists only one annotation function $a_M$. 
%\end{lemma}
%\begin{proof}
%    We proof Lemma \ref{lemma:2_17} by induction.
%    Consider any root-to-leaf path $p$ of $M$ of length $k$. 
%    For the base case $k = 1$, $p$ only contains a root vertex $v_r$. 
%    By Eqn.~\ref{eqn:constrained}, there only exists one $a_M$ of $v_r$ and $a_M(v_r) = d(v_r)$ as there does not exist a parent vertex $u$ of the root vertex $v_r$ in $p$.
%    For the induction step, assume that $p$ of length $k > 1$ only has one annotation function.
%    We extend $k$ to $k+1$ by adding one child vertex $v_i$ to the leaf vertex $v_l$ of $p$. 
%    As there must exist a parent vertex $v_l$ for $v_i$, $a_M(v_i)$ is determined by whether $a_M(v_l) \in r(v_i)$ as defined in Eqn.~\ref{eqn:constrained}. 
%    Therefore, $v_i$ in $M$ has exactly one $a_M$, and by mathematical induction, there exists only one $a_M$ for a given $r$ and $M$.  
%\end{proof}

%\begin{proof}
%    We proof Lemma \ref{lemma:2_17} by induction. 
%    Consider the base case where the vertex $v_i$ is the root of $M$. 
%    By Eqn.~\ref{eqn:constrained}, there only exists one $a_M$ of $v_i$ and $a_M(v_i) = d(v_i)$ as there does not exist a parent vertex $u$ of the root vertex $v_i$. 
%    For the induction step, let $v_j$ be any vertex following the root $v_i$ in any root-to-leaf path $p$ of $M$. 
%    For each $v_j$, there must exist a parent vertex $v_k$ of $v_j$ in $p$ as $v_j$ follows the root $v_i$ in $p$, and $a_M(v_j)$ is determined by whether $a_M(v_k) \in r(v_j)$, as defined in Eqn.~\ref{eqn:constrained}. 
%    Therefore, any subsequent vertices of the root $v_i$ in $M$ have exactly one $a_M$. 
%    Hence, there exists only one $a_M$ for a given $r$ and $M$. 
%\end{proof}

%\ms{Lemma: given a replication function $r$ and a match $M$ there is only one constrained annotation function $a_M$ since the mapping of each vertex to a replica is constrained by Eqn.~\ref{eqn:constrained}. You start from the root, which has only one choice. Then for each path $p$ in the $C_M$ you have that for each parent-child pair $(v,u)$ given $a_M(v)$ and $r$ then $a_M(u)$ is determined by the equation.}
%\ms{ Then argue in the text that the min part in Def 2.9 is eliminated.}
%\nn{Done. }

%In the running example, the query executor first processes $v_2$ at $s_1$. 
%As the next hop $v_4$ does not exist locally, the query executor routes the subquery to the server $s_2$ that contains the master copy of $v_4$. 
%After processing $v_4$ at $s_2$, the replica of $v_6$ can be found locally, therefore, $l_Q = l(s_1,s_2) = 1$. 

==> sections/system_architecture.tex <==
\section{System Architecture}
\begin{figure}[ht]
  \centerline{\includegraphics[width=0.45\textwidth]{figures/system_architecture.pdf}}
  \caption{Proposed system architecture}
\label{fig:system_architecture}
\end{figure}

\nn{do we actually need a system arcihtecture? We are not proposing a new system. We are more like proposing a replication algorithm. }

